Learning State-Aware Visual Representations from Audible Interactions

We propose a self-supervised algorithm to learn representations from egocentric video data. Recently, significant efforts have been made to capture humans interacting with their own environments as they go about their daily activities. In result, several large egocentric datasets of interaction-rich multi-modal data have emerged. However, learning representations from videos can be challenging. First, given the uncurated nature of long-form continuous videos, learning effective representations require focusing on moments in time when interactions take place. Second, visual representations of daily activities should be sensitive to changes in the state of the environment. However, current successful multi-modal learning frameworks encourage representation invariance over time. To address these challenges, we leverage audio signals to identify moments of likely interactions which are conducive to better learning. We also propose a novel self-supervised objective that learns from audible state changes caused by interactions. We validate these contributions extensively on two large-scale egocentric datasets, EPIC-Kitchens-100 and the recently released Ego4D, and show improvements on several downstream tasks, including action recognition, long-term action anticipation, and object state change classification.

==> latex/0-abstract.tex <==
\begin{abstract}
We propose a self-supervised algorithm to learn representations from egocentric video data. Recently, significant efforts have been made to capture humans interacting with their own environments as they go about their daily activities. In result, several large egocentric datasets of interaction-rich multi-modal data have emerged. However, learning representations from videos can be challenging. 
First, given the uncurated nature of long-form continuous videos, learning effective representations require focusing on moments in time when interactions take place. Second, visual representations of daily activities should be sensitive to changes in the state of the environment. However, current successful multi-modal learning frameworks encourage representation invariance over time.
To address these challenges, we leverage audio signals to identify moments of likely interactions which are conducive to better learning. We also propose a novel self-supervised objective that learns from audible state changes caused by interactions. We validate these contributions extensively on two large-scale egocentric datasets, \epickitchens and the recently released Ego4D, and show improvements on several downstream tasks, including action recognition, long-term action anticipation, and object state change classification.
\end{abstract}

==> latex/00_space_saving.tex <==
%% Make everything look better.
%% http://tex.stackexchange.com/questions/553/what-packages-do-people-load-by-default-in-latex
%% http://www.howtotex.com/packages/9-essential-latex-packages-everyone-should-use/
\usepackage{microtype}

%% Shrink space around figures.
%% This beats manually adding negative \vspace commands everywhere.
% \setlength{\textfloatsep}{0pt}
% \setlength{\textfloatsep}{20pt plus 2pt minus 4pt}
\setlength{\textfloatsep}{16pt plus 2pt minus 4pt}
% \setlength{\textfloatsep}{6pt plus 2pt minus 4pt}
% \setlength{\dbltextfloatsep}{0pt}
% \setlength{\intextsep}{0pt}
\setlength{\abovecaptionskip}{4pt}
\setlength{\belowcaptionskip}{1pt}
% \setlength{\parskip}{0pt}
%% around equations
% \setlength{\abovedisplayskip}{1pt}
% \setlength{\belowdisplayskip}{1pt}
% \setlength\abovedisplayshortskip{1pt}
% \setlength\belowdisplayshortskip{1pt}

%% The wrapfigure environment is also a good way to use less space for a small figure.
%% It is finicky.
%% See: http://en.wikibooks.org/wiki/LaTeX/Floats,_Figures_and_Captions#Wrapping_text_around_figures

%% Shrink space around enumerate and itemize
%% From: http://tex.stackexchange.com/questions/10684/vertical-space-in-lists
%\usepackage{enumitem}
%% Set it globally:
% \setlist{nosep} % or \setlist{noitemsep} to leave space around whole list
% \setlist{itemsep=1pt, topsep=3pt}
%% Or locally:
% \begin{enumerate}[itemsep=1pt, topsep=12pt, partopsep=0pt]

%% Less space around titles.
%% From: http://tex.stackexchange.com/questions/4999/change-whitespace-above-and-below-a-section-heading
% \usepackage[medium,compact]{titlesec}
%% or
% \usepackage{titlesec}
% \titlespacing*{\section}{0pt}{*1}{*1}

%% Shrink the \paragraph command.
% \renewcommand{\paragraph}[1]{\noindent {\bf #1}}

%% Allow Latex to use a smaller minimum spacing between lines.
%\renewcommand{\baselinestretch}{0.97}
% \renewcommand{\baselinestretch}{0.99}

%% Shrink space between lines. You probably want to prefer baselinestretch in general.
%% From: http://tex.stackexchange.com/questions/23824/6-lines-in-one-inch
%% 6 lines in one inch with an 11pt font:
% \linespread{0.990}
%\linespread{0.909}
%\linespread{1}

%% Shrink the spacing between lines in just the bibliography. This is good.
% \usepackage{setspace}

%% Then wrap the bibliography in a \begin{spacing}. You can wrap any section like this.
% \begin{spacing}{0.9}
% \bibliographystyle{...}
% \bibliography{refe

==> latex/1-intro-bkp.tex <==
\section{Introduction}

% Representation learning for daily activities
Recall the last time you cooked. You may have picked ingredients from the fridge, cut vegetables, stir fried them in a pan, grilled a steak, and washed the dishes. In the process, you have interacted with many different objects causing them to change, oftentimes irreversibly.
Visual understanding of our environments thus requires learning representations that are sensitive to the actions we take, the objects we interact with, and the changes in their state we cause.
With the goal of developing models capable of such fine-grained understanding, major efforts have been made to capture humans interacting with their own environments as they go about their daily activities~\cite{damen2020rescaling, grauman2021ego4d}. 
% However, densely annotating these egocentric videos can be costly and painstakingly slow. 
In this work, we ask the question, `What can be learned from such interaction-rich, multi-modal, egocentric data without human supervision?' 
% In particular, we tackle the challenges introduced by the untrimmed nature of egocentric datasets, and propose a novel self-supervised objective that focuses on interactions in the environment and state changes.

% Detecting moments of interaction to help learning from untrimmed data through self-supervision
Recent developments in self-supervised learning have shown that contrastive learning techniques learn strong representations without the need for human annotations~\cite{simclr,byol,cpc,moco,swav}. 
However, despite not directly relying on human annotations, video-based contrastive methods are designed to leverage carefully trimmed clips, displaying a single action or object interaction. This is in contrast to real-world data where video data is predominantly untrimmed. Learning from untrimmed video poses a major challenge, as a significant portion of the data does not focus on the concepts we want to learn.


To address this problem, we propose \textbf{M}oment of \textbf{I}nteraction-guided \textbf{A}udio-\textbf{V}isual \textbf{R}epresentation \textbf{L}earning~(MoI-AVRL). In MoI-AVRL, we search for audio cues that are indicative of moments in time when interactions or object state changes occur. Consider, for example, the acts of opening a fridge or placing a pan on the stove. Actions like these create clear and consistent sound signatures due to the collision and/or physical interaction between objects. These moments can be easily detected from audio alone, and can be used to target training on interesting portions of the untrimmed videos. In fact, we show in MoI-AVRL that even simple handcrafted spectrogram-based approaches are sufficient to identify interesting moments in time, and that representation learning benefits substantially by using them to sample training clips.

% Audio visual learning in egocentric data
In addition to sampling, the audio content in egocentric data can also be used as a target for representation learning, as audio is highly informative of the type of interactions taking place. The correlation between audio and visual signals have been extensively studied to learn general video representations~\cite{}. In this paper, we also leverage audio-visual association techniques~\cite{} for training MoI-AVRL via self-supervised learning, and show that audio is a strong supervisory signal for egocentric data as well. 

% State change self-supervision
By mapping co-occurring visual and audio signals into the same feature space, MoI-AVRL learns to distinguish objects by the sounds they make. However, optimizing for audio-visual associations does not encourage the learned representations to be informative of their states (\eg, representations that can distinguish between closed and opened fridge, or vegetables before and after chopping them). To better capture these state changes, we introduce a novel audio-visual self-supervised objective called Audible State Change (\loss) loss, in which audio representations at key moments in time are required to be informative of the \textit{change} in the corresponding visual representations over time. The intuition behind this objective is that transitions between object states are often marked by characteristic sounds. Thus, models optimized under this objective would associate the distinct sounds not only with the objects themselves (as accomplished with contrastive approaches), but also with the transition between two different states of the object. 

In sum, the major contributions of this work are the following:
\begin{itemize}
    \item We introduce MoI-AVRL to leverage audio signals to effectively identify moments in time within long untrimmed data that are conducive to better self-supervised learning.
    \item We introduce a novel audio-visual self-supervised objective called Audible State Change (\loss) loss that is designed to capture state changes, and show that this objective is complementary to audio-visual associations.
    \item We validate these contributions extensively on two egocentric datasets, EPIC-Kitchens-100~\cite{damen2020rescaling} and the recently released Ego4D~\cite{grauman2021ego4d}, where we demonstrate the benefits of \method for several downstream tasks, including action recognition, long term action anticipation, and object state change classification.
\end{itemize}

%%%%% Himangi
% The world of internet and social networking is contributing to multimodal audio-visual data at an ever increasing pace. In the recent years, several self-supervised techniques have emerged to learn from this multimodal data without requiring any annotations. Such techniques can train the model to learn effective representations without any supervision which can be later used to achieve state-of-the-art performance on downstream tasks. 

% To the best of our knowledge, the existing audio-visual self-supervised techniques are designed to leverage trimmed videos optimally where a single video clip has a duration of less than a minute and only exhibit a single action. But real-world videos are predominantly untrimmed where the duration of a single video can be several minutes and beyond, and each video can exhibit several actions happening one after the other (with actions even overlapping each other). Moreover, the nature of an untrimmed setting leads to the sequence of actions to happen in the same or gradually changing spatial setting. At the same time, actions can have a strong temporal relationship, can be semantically related to each other and can happen only in a certain temporal order (eg. in epic kitchen dataset…). On the contrary, actions across a set of trimmed videos are independent of each other and usually have a high spatial disparity. These difference limit the existing audio-visual self-supervised methods to perform optimally on downstream tasks comprising untrimmed videos. 

% Figure <> illustrates such untrimmed videos from an egocentric kitchen setting. We can observe that there is a sharp audio peak wherever there is a change in action visually. Moreover, the consecutive actions are visually quite similar but at the same time, exhibit a natural temporal order (such as opening of fridge followed by closing it). Leveraging these observations, we propose SSRL (Simultaneous Segmentation and Representation Learning). SSRL uses locations in a video with high audio prominence as indicator of change in the action and learns representations that distinguishes the visual information before and after such peaks. Moreover, it proposes a novel loss objective that learns to correlate the visual temporal order of features with the corresponding audio information. 


% learn the correct representation of action, closing and opening fridge, two actions would be indistinguishable, learn a representation that is capable of distinguishing actions such as closing and opening fridge, when visually they are quite similar, if we apply typical contrastive, aot loss - audio information helps in deciding order and also helpful for fine-grained actions. when we don't have access to the information. ; order prediction based on audio

% untrimmed video has many action, state separation, related to an action, before and after state defined by the audio peak, our method learns the state representation of specific action. Specific action has a before and after state. 

% \textbf{Why do we need this algorithm?}
% Previous methods 

% \textbf{when will this algorithm be required?}
% we perform a more detailed and in-grained analysis for detecting actions. 

% \textbf{How improving on other methods?}


% \textbf{any challenge that this method solves?}


% \textbf{3 point technical contributions}
% Contributions
% 1) fine-grained action recognition
% 2) leverage audio, multi-modal
% 3) show results on ego-centric datasets.
% 4) untrimmed videos
% 5) ours is the first method to explore fine-grained action recognition in a self-supervised manner. Previous methods have explored transformers.

% \textbf{what the old methods do?}

% (fig 1. State 1 (full vegetable), Audio Peak, State 2 (cut vegetable))

% Novelty on fine-grained action recognition: Recently, methods have shown the application of contrastive learning on videos and show their results on the downstream task of action recognition. However, previous methods classify a video clip having only one action label. 

% State change: Previous methods use the visual clip as one, however, we make a more detailed analysis by treating the state before and after an action as different. 

% 1. This will help to better understand a specific action by knowing the uniqueness of action. For each action, the before and after state is different which will lead to different visual features and unique features for that specific action.
% 2. every action has a unique sound associated with it. We try to leverage that audio information. 

% We try to achieve this by leveraging the audio modality. We hypothesize that when there is a change in action, there is a change in the visual state. For example, for a action of cutting of vegetables, the chopping sounds shows a transition from the full vegetable to a cut vegetable. This transition in state has a change of visual features. Overall, this can be leveraged in detecting multiple action in a video clip and to do a fine-grained action recognition.

% Other methods only use the visual modality and do not use the audio modality, however, we show that audio modality has important information for detecting the change in actions and doing fine-grained action recognition. 

% The method which use audio treat the audio before and after action in the same way. However, we explore the visual and audio states before and after an action.

% 1. to address the challenge that the videos available in the wild are untrimmed videos with multiple action and no easy to chop it into trimmed videos and divide it. we are not able to leverage se
% self-super needs a lot of data, leveraging such dataset is challenging,need to be properly curated.
% Previous works assume a single action in their clip. They assume a trimmed video setting with a single action in their clip. No paper so far that can leverage on the wild untrimmed videos which has a continuous stream of different actions. and given the kind of videos we find on social media, multi media, it is important that we need to have the ability that there is only one action. 
% our algorithm can learn from untrimmed videos in a self-supervised manner. 

% 2. when action happens, audio has a peak, using those peaks to figure out the separation, video has separate states, and we leverage that. 

% a). task
% b). algorithm
% c). better results


% \textbf{(Does our algorithm have any component which is specialized to ego centric dataset?)}
% We test our method on challenging ego-centric datasets having untrimmed videos which presents more challenges than the conventional third-person videos.
% defines the change in action by leveraging audio modality. 
% We try to explore self-supervised contrastive learning on ego-centric datasets.



% \textbf{2. state of the art performance on epic kitchens-100 self supervised method. 
% 3. what's the difference between action recognition, classification, detection, video recognition?}

% Introduction
% There are exisitng AV learning methods, but the problem 
% You are proposing a AV learning method that can be more effective on untrimmed videos. Untrimmed videos have change of states in the action, the network may not be able to learn in a better way, audio information to figure out the change of state. We propose a novel self-supervised objective.
% Current AV are not effective even in the presence of action segments in untrimmed videos.


==> latex/1-introback.tex <==


\section{Introduction}

% Representation learning for daily activities
Recall the last time you cooked. You may have picked ingredients from the fridge, cut vegetables, stir fried them in a pan, grilled a steak, and washed the dishes. In the process, you have interacted with many different objects causing them to change, oftentimes irreversibly.
Visual understanding of our environments thus requires learning representations that are sensitive to the actions we take, the objects we interact with, and the changes in their state we cause.
With the goal of developing models capable of such fine-grained understanding, major efforts have been made to capture humans interacting with their own environments as they go about their daily activities~\cite{damen2020rescaling, grauman2021ego4d}. 
% However, densely annotating these egocentric videos can be costly and painstakingly slow. 
In this work, we ask the question, `What can be learned from such interaction-rich, multi-modal, egocentric data without human supervision?' 
% In particular, we tackle the challenges introduced by the untrimmed nature of egocentric datasets, and propose a novel self-supervised objective that focuses on interactions in the environment and state changes.

% Detecting moments of interaction to help learning from untrimmed data through self-supervision
Recent developments in self-supervised learning (SSL)~\cite{cpc,simclr,moco,byol} has brought into question the need for human annotations in order to learn strong visual representations.
However, despite not directly relying on human annotations, current state-of-the-art SSL methods for multi-modal data~\cite{alwassel2020self, morgado2021audio, brave} are designed to leverage carefully selected clips, displaying a single action or object interaction. 
This is in contrast to the predominantly \textit{untrimmed} real-world data characteristic of large egocentric datasets of daily activities. Here, unlike action centric datasets, the most `interesting` or `interaction-rich` clips have NOT been carefully selected by human annotators. Thus, learning from untrimmed video poses a major challenge, as a significant portion of the data does not focus on the concepts we want to learn.



To address this problem, we propose to focus learning on moments in time where interactions are likely to occur. Consider, for example, the acts of opening a fridge or placing a pan on the stove. Actions like these create clear and consistent sound signatures due to the physical interaction between objects. These moments can also be easily detected from audio alone, and can be used to target training on interesting portions of the untrimmed videos. We show that even a simple spectrogram-based handcrafted detector is sufficient to identify interesting moments in time, and that representation learning benefits substantially from using them to sample training clips.

% State change self-supervision
In interaction rich environments, audio is a strong target for self-supervised visual representation learning, as it is highly informative of the type of interactions taking place. For example, consider again the cooking scene described above. You would likely recognize most of the activities taking place, even without looking, from the opening and close of the fridge, to cutting and cooking, and washing the dishes.
Prior work on audio-visual correspondence~\cite{} use the natural co-occurrence of sounds and the visual manifestations of their sources as the source of supervision.
However, optimizing for audio-visual correspondence does not encourage the learned representations to be informative of object states (\eg, representations that can distinguish between closed and opened fridge, or vegetables before and after chopping them). To better capture state changes, we introduce a novel audio-visual self-supervised objective called Audible State Change (\loss) loss, in which audio representations at key moments in time are required to be informative of the \textit{change} in the corresponding visual representations over time. The intuition behind this objective is that transitions between object states are often marked by characteristic sounds. Thus, models optimized under this objective would associate the distinct sounds not only with the objects themselves (as accomplished with contrastive approaches), but also with the transition between two different states of the object. 

In sum, the major contributions of this work are the following.
We introduce \todo{method} \method -- a self-supervised algorithm for representation learning from videos of audible interactions. \method uses the audio signals in two unique ways: (1) to identify moments in time within long untrimmed data that are conducive to better self-supervised learning and (2) to learn representations that focus on the visual state changes caused by audible interactions. We validate these contributions extensively on two egocentric datasets, EPIC-Kitchens-100~\cite{damen2020rescaling} and the recently released Ego4D~\cite{grauman2021ego4d}, where we demonstrate the benefits of \method for several downstream tasks, including action recognition, long term action anticipation, and object state change classification.
% \begin{itemize}
%     \item We introduce \todo{method} \method -- a new self-supervised 
%     to leverage audio signals to effectively identify moments in time within long untrimmed data that are conducive to better self-supervised learning.
%     \item We introduce a novel audio-visual self-supervised objective called Audible State Change (\loss) loss that is designed to capture state changes, and show that this objective is complementary to audio-visual associations.
%     \item We validate these contributions extensively on two egocentric datasets, EPIC-Kitchens-100~\cite{damen2020rescaling} and the recently released Ego4D~\cite{grauman2021ego4d}, where we demonstrate the benefits of \method for several downstream tasks, including action recognition, long term action anticipation, and object state change classification.
% \end{itemize}

%%%%% Himangi
% The world of internet and social networking is contributing to multimodal audio-visual data at an ever increasing pace. In the recent years, several self-supervised techniques have emerged to learn from this multimodal data without requiring any annotations. Such techniques can train the model to learn effective representations without any supervision which can be later used to achieve state-of-the-art performance on downstream tasks. 

% To the best of our knowledge, the existing audio-visual self-supervised techniques are designed to leverage trimmed videos optimally where a single video clip has a duration of less than a minute and only exhibit a single action. But real-world videos are predominantly untrimmed where the duration of a single video can be several minutes and beyond, and each video can exhibit several actions happening one after the other (with actions even overlapping each other). Moreover, the nature of an untrimmed setting leads to the sequence of actions to happen in the same or gradually changing spatial setting. At the same time, actions can have a strong temporal relationship, can be semantically related to each other and can happen only in a certain temporal order (eg. in epic kitchen dataset…). On the contrary, actions across a set of trimmed videos are independent of each other and usually have a high spatial disparity. These difference limit the existing audio-visual self-supervised methods to perform optimally on downstream tasks comprising untrimmed videos. 

% Figure <> illustrates such untrimmed videos from an egocentric kitchen setting. We can observe that there is a sharp audio peak wherever there is a change in action visually. Moreover, the consecutive actions are visually quite similar but at the same time, exhibit a natural temporal order (such as opening of fridge followed by closing it). Leveraging these observations, we propose SSRL (Simultaneous Segmentation and Representation Learning). SSRL uses locations in a video with high audio prominence as indicator of change in the action and learns representations that distinguishes the visual information before and after such peaks. Moreover, it proposes a novel loss objective that learns to correlate the visual temporal order of features with the corresponding audio information. 


% learn the correct representation of action, closing and opening fridge, two actions would be indistinguishable, learn a representation that is capable of distinguishing actions such as closing and opening fridge, when visually they are quite similar, if we apply typical contrastive, aot loss - audio information helps in deciding order and also helpful for fine-grained actions. when we don't have access to the information. ; order prediction based on audio

% untrimmed video has many action, state separation, related to an action, before and after state defined by the audio peak, our method learns the state representation of specific action. Specific action has a before and after state. 

% \textbf{Why do we need this algorithm?}
% Previous methods 

% \textbf{when will this algorithm be required?}
% we perform a more detailed and in-grained analysis for detecting actions. 

% \textbf{How improving on other methods?}


% \textbf{any challenge that this method solves?}


% \textbf{3 point technical contributions}
% Contributions
% 1) fine-grained action recognition
% 2) leverage audio, multi-modal
% 3) show results on ego-centric datasets.
% 4) untrimmed videos
% 5) ours is the first method to explore fine-grained action recognition in a self-supervised manner. Previous methods have explored transformers.

% \textbf{what the old methods do?}

% (fig 1. State 1 (full vegetable), Audio Peak, State 2 (cut vegetable))

% Novelty on fine-grained action recognition: Recently, methods have shown the application of contrastive learning on videos and show their results on the downstream task of action recognition. However, previous methods classify a video clip having only one action label. 

% State change: Previous methods use the visual clip as one, however, we make a more detailed analysis by treating the state before and after an action as different. 

% 1. This will help to better understand a specific action by knowing the uniqueness of action. For each action, the before and after state is different which will lead to different visual features and unique features for that specific action.
% 2. every action has a unique sound associated with it. We try to leverage that audio information. 

% We try to achieve this by leveraging the audio modality. We hypothesize that when there is a change in action, there is a change in the visual state. For example, for a action of cutting of vegetables, the chopping sounds shows a transition from the full vegetable to a cut vegetable. This transition in state has a change of visual features. Overall, this can be leveraged in detecting multiple action in a video clip and to do a fine-grained action recognition.

% Other methods only use the visual modality and do not use the audio modality, however, we show that audio modality has important information for detecting the change in actions and doing fine-grained action recognition. 

% The method which use audio treat the audio before and after action in the same way. However, we explore the visual and audio states before and after an action.

% 1. to address the challenge that the videos available in the wild are untrimmed videos with multiple action and no easy to chop it into trimmed videos and divide it. we are not able to leverage se
% self-super needs a lot of data, leveraging such dataset is challenging,need to be properly curated.
% Previous works assume a single action in their clip. They assume a trimmed video setting with a single action in their clip. No paper so far that can leverage on the wild untrimmed videos which has a continuous stream of different actions. and given the kind of videos we find on social media, multi media, it is important that we need to have the ability that there is only one action. 
% our algorithm can learn from untrimmed videos in a self-supervised manner. 

% 2. when action happens, audio has a peak, using those peaks to figure out the separation, video has separate states, and we leverage that. 

% a). task
% b). algorithm
% c). better results


% \textbf{(Does our algorithm have any component which is specialized to ego centric dataset?)}
% We test our method on challenging ego-centric datasets having untrimmed videos which presents more challenges than the conventional third-person videos.
% defines the change in action by leveraging audio modality. 
% We try to explore self-supervised contrastive learning on ego-centric datasets.



% \textbf{2. state of the art performance on epic kitchens-100 self supervised method. 
% 3. what's the difference between action recognition, classification, detection, video recognition?}

% Introduction
% There are exisitng AV learning methods, but the problem 
% You are proposing a AV learning method that can be more effective on untrimmed videos. Untrimmed videos have change of states in the action, the network may not be able to learn in a better way, audio information to figure out the change of state. We propose a novel self-supervised objective.
% Current AV are not effective even in the presence of action segments in untrimmed videos.


==> latex/1-introduction.tex <==
\section{Introduction}
Recent successes in self-supervised learning (SSL)~\cite{cpc,simclr,moco,byol} has brought into question the need for human annotations in order to learn strong visual representations. However, current approaches are bottlenecked by the lack of rich data -- they learn from static images which lack temporal information and restrict the ability to learn object deformations and state changes. It is clear that we need videos to learn rich representations in self-supervised manner.

Learning representations from videos is however quite challenging. The first challenge is choosing the right SSL loss. Approaches such as ~\cite{wang2015unsupervised, purushwalkam2020aligning} have attempted to learn representations that are invariant to object deformations/viewpoints. However, many downstream tasks require representations that are sensitive to these deformations. Another alternative has been to use the multi-modal data~\cite{alwassel2020self, morgado2021audio, brave} and learn representations via audio. But again most of these approaches seek to align audio and visual features in a common space, leading to invariant representations as well. The second challenge is dealing with the fact that current video-based SSL approaches exploit the curated nature of video datasets, such as Kinetics~\cite{carreira2017quo}. These approaches are designed to leverage carefully selected clips, displaying a single action or object interaction. This is in contrast to the predominantly \textit{untrimmed} real-world data characteristic of large egocentric datasets of daily activities. Here, unlike action centric datasets, the most `interesting` or `interaction-rich` clips have NOT been carefully selected by human annotators. Thus, learning from untrimmed video poses a major challenge, as a significant portion of the data does not focus on the concepts we want to learn.

In this work, we ask the question, `Can we learn meaningful representations from interaction-rich, multi-modal streams of egocentric data?' 
Learning from continuous streams of data requires focusing on the right moments when the actual interactions are likely to occur. Consider, for example, the acts of opening a fridge or placing a pan on the stove. Actions like these create clear and consistent sound signatures due to the physical interaction between objects. These moments can be easily detected from audio alone and can be used to target training on interesting portions of the untrimmed videos. We show that even a simple spectrogram-based handcrafted detector is sufficient to identify interesting moments in time, and that representation learning benefits substantially from using them to sample training clips.

But what should the loss be? Prior work on audio-visual correspondence (AVC)~\cite{de1994learning,arandjelovic2017look,morgado2021audio} uses the natural co-occurrence of sounds and the visual manifestations of their sources as the source of supervision. However, since the AVC objective still favors invariance, the learned representations are not informative of the changes that happen over time (\eg, representations that can distinguish between closed and opened fridge, or vegetables before and after chopping them). To better capture state changes, we introduce a novel audio-visual self-supervised objective, in which audio representations at key moments in time are required to be informative of the \textit{change} in the corresponding visual representations over time. The intuition behind this objective is that transitions between object states are often marked by characteristic sounds. Thus, models optimized under this objective would associate the distinct sounds not only with the objects themselves (as accomplished with AVC), but also with the transition between two different states of the object. 

To this end, we introduce \method~--~\textbf{Rep}resentation \textbf{L}earning from \textbf{A}udible \textbf{I}nteractions, a self-supervised algorithm for representation learning from videos of audible interactions. \method uses the audio signals in two unique ways: (1) to identify moments in time that are conducive to better self-supervised learning and (2) to learn representations that focus on the visual state changes caused by audible interactions. We validate these contributions extensively on two egocentric datasets, \epickitchens~\cite{damen2020rescaling} and the recently released Ego4D~\cite{grauman2021ego4d}, where we demonstrate the benefits of \method for several downstream tasks, including action recognition, long term action anticipation, and object state change classification.

\begin{figure}[t!]
    \centering
    \includegraphics[trim=0 0 2cm 0, clip, width=\linewidth]{figures/teaserv10.pdf}
    \vspace{-5mm}
    \caption{\textbf{Moments of audible interactions in a long, untrimmed video.} 
    Random moments in time are likely to contain NO interactions, \eg, timestamp shown by the \textcolor{gray}{gray} box. Since no interactions occur, no changes in the before and after states are observed. By sampling from moments of interaction~(MoI), as shown in the \textcolor{red}{red} box, we can learn representations that are sensitive to the change in the visual state caused by interactions. }
    \label{fig:intro}
\end{figure}

==> latex/2-related.tex <==
\section{Related Work}

\textbf{Self-supervised learning.} Self-supervised learning methods operate on an unlabeled dataset by explicitly defining pretext tasks such as solving jigsaw puzzle~\cite{jigsaw}, patch location prediction~\cite{doersch2015unsupervised}, inpainting~\cite{inpainting}, and image rotation~\cite{rotation} prediction. Following these, the next wave of self-supervised methods has been based on contrastive learning that learns representations with the help of data augmentation and instance discrimination~\cite{simclr,byol,cpc,moco,swav}. These methods have shown rapid progress in self-supervised learning for images. While these approaches explore the spatial information of images, \method leverages the temporal information of videos.

\textbf{Video representation learning.} Relevant to our proposed approach is self-supervised representation learning for videos where the spatiotemporal pretext tasks are designed such as temporal order prediction~\cite{misra2016shuffle,videocliporder,spacetimecubic,aot}, predicting motion and appearance statistics~\cite{motionappeareance}, pace prediction~\cite{pace}, temporal cycle consistency~\cite{temporalcycle, cyclecorrespondence}, and video colorization~\cite{videocolorization}. Contrastive learning has also been widely adopted in the domain of video~\cite{cvrl, cotrain, contrastorder, brave, zeng2021contrastive, han2020memory, feichtenhofer2021large} with impressive results on action recognition tasks. These methods however learn representations that are invariant to spatio-temporal augmentations, such as temporal jittering, and thus are incapable of representing object state changes. Closer to the objective of \method, we include relevant literature on audio-visual representation learning from videos, where the audio stream is additionally utilized. 


\textbf{Audio-visual representation learning.} 
Learning without additional supervision has also been explored in the context of the audio modality with the help of audio-visual correspondence (AVC)~\cite{arandjelovic2017look, objectsthatsound}. As stated simply, AVC is the binary classification task of predicting if a video clip and a short audio clip correspond with each other or not (details in \cref{sec:avc}). Similar tasks like temporal synchronization~\cite{korbar2018cooperative, owens2018audio} between audio and video, audio classification~\cite{asano2020labelling, alwassel2020self, chung2019perfect}, 
% Bookmark - UJ
spatial alignment prediction between audio and 360-degree videos~\cite{morgado2020learning} have been shown beneficial for learning effective multi-modal video representations. Other works explore contrastive learning for both audio and video modality~\cite{morgado2021audio, patrick2020multi, morgado2021robust} as a cross-modal instance discrimination task. 

\textbf{Fine-grained video understanding.} 
Real-world videos are often untrimmed in nature and have multiple actions in a single video. Along this line, fine-grained analysis has been studied for videos in the form of a query-response temporal attention mechanism~\cite{zhang2021temporal}, bi-directional RNN~s\cite{singh2016multi}, and semi-supervised learning problem ~\cite{doughty2022you}. While these works only utilize the visual modality, another line of work has also explored multi-modal fine-grained video understanding as a transformer-based model~\cite{kazakos2021little} or by exploiting the correspondence between modalities~\cite{munro2020multi}. In our work, we try to conduct fine-grained video understanding in a self-supervised manner.

\textbf{Egocentric datasets.} 
Egocentric datasets offer new opportunities to learn from a first-person point of view, where the world is seen through the eyes of an agent. Many egocentric datasets have been developed such as Epic-kitchens~\cite{Damen2018EPICKITCHENS, damen2020rescaling} which consist of daily activities performed in a kitchen environment, Activities of Daily Living~\cite{pirsiavash2012detecting}, UT Ego~\cite{lai2014unsupervised, su2016detecting}, the Disney Dataset~\cite{fathi2012social}, and the recently released large-scale Ego4D dataset~\cite{grauman2021ego4d} which consists of day-to-day life activities in multiple scenarios such as household, outdoor spaces, workplace, etc. Multiple challenges and downstream tasks have explored for egocentric datasets like action recognition~\cite{kazakos2021little, kazakos2019epic, li2021ego}, action localization~\cite{ramazanova2022owl}, action anticipation~\cite{girdhar2021anticipative, singh2016krishnacam, liu2019forecasting, abu2018will, furnari2020rolling}, human-object interactions~\cite{nagarajan2019grounded, damen2014you, cai2018understanding}, parsing social interactions~\cite{ng2020you2me}, and domain adaptation~\cite{munro2020multi}. In our work, we evaluate the efficiency of the representations learned by our self-supervised approach on the \epickitchens and Ego4D datasets over multiple downstream tasks.


==> latex/3-methods.tex <==
\vspace{-2mm}
\section{\method}
\vspace{-2mm}
% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=\linewidth]{figures/teaserv4.pdf}
%     \caption{\textbf{Moment of Interaction~(MoI) aligning with the state change} For a given video clip and its corresponding spectrogram, a random timestamp is sampled as shown by the \textcolor{gray}{gray} box on the spectrogram. We observe that there is no change in the before and after state at this timestamp. However, when we sample a moment of interaction~(MoI) as shown in the \textcolor{red}{red} box, we observe a change in the before and after state of the object.\label{fig:intro}}
% \end{figure}
In this section, we detail our approach to learn audio-visual representations from and for interaction-rich egocentric data in a self-supervised manner, \ie, without relying on human annotated labels. 
\cref{sec:overview} provides an overview of \method and motivates the two key contributions of this work -- identifying `moments of interaction' (MoI) and learning from `audible visual state changes'. \cref{sec:moi} details the proposed approach for MoI detection and section \cref{sec:stc} explains the proposed self-supervised objective for learning state-aware representations. \cref{sec:avc} explains the objective of audio-visual correspondence learning used to train \method. \cref{sec:learning} brings both objectives together and includes necessary details for reproducibility.
% from   towards  necessary preliminaries on audio-visual correspondence learning, a standardized framework for audio-visual representation learning. Next, we give . Finally, we highlight two challenges that arise when learning from untrimmed egocentric data -- identifying `moments of interaction' and learning `state-aware representations' -- and interleave our proposed solutions to tackle these challenges. 
\vspace{-1mm}
% Baseline
\subsection{Overview}
\label{sec:overview}
Given a dataset $\Dcal=\{(v_i, a_i)_{i=1}^N\}$ containing $N$ long (untrimmed) audio-visual streams, our goal is to learn visual and audio encoders, denoted $f_V$ and $f_A$, that can effectively represent egocentric data.
An overview of the proposed approach is depicted in \cref{fig:system}. 
For each sample $(v, a) \in \Dcal$, we search for moments of interaction (MoI) using the audio stream, and extract short audio and visual clips around these MoI. These trimmed clips are then encoded into a vectorized representation using $f_V$ and $f_A$. The whole system is trained to optimize two self-supervised losses -- an audio-visual correspondence loss $\Lavc$, and a novel self-supervised loss that learns from audible state changes $\Lastc$.

\textit{Why detect moments of interaction (MoI)?}
Untrimmed video of daily activities often contains long periods without interactions, which aren't useful for training. Instead, we search for moments in time that are more likely to contain interactions which we refer to as moments of interaction (MoI).

% Untrimmed videos of daily activities contain long periods without any interaction. We hypothesize that these non-interactive periods are not useful for training. Instead, we search for moments in time that are more likely to have egocentric interactions. To do this without any labeled supervision, we find the audio stream to be helpful.

\textit{Why learn from audible state changes?}
Visual representations of daily activities should be informative of the state of the environment and/or objects being interacted with. Moreover, changes in the environment are usually caused by physical interactions, which produce distinct sound signatures. We hypothesize that state-aware representations can be obtained by learning to associate audio with the change of visual representation during a moment of interaction.

% Previous version:
% ---------
% \textit{Why MoI?} Untrimmed video of daily activities often contains long periods without interactions. We hypothesize that these portions are not useful for training, and instead search for moments in time that are more likely to contain interactions.

% \textit{Why learning from audible state changes?}
% Visual representations of daily activities should be informative of the state of the environment and/or objects within it. Since changes in the environment are often caused by physical interactions, which can produce distinct sound signatures, we hypothesize that state-aware representations can be obtained by learning to associate audio with the change of visual representation during a moment of interaction.
% ---------

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/system.pdf}
    \caption{\textbf{Overview of \method.} \method seeks to learn audio and visual encoders ($f_A$ and $f_V$) by (1) detecting and focusing training data on moments of interaction (MoI) present in untrimmed videos and (2) solving a combination of two tasks -- audio-visual correspondence (\avc) and audio identifiable state changes (\loss).}
    \label{fig:system}
\end{figure}


% MOI detection
\subsection{Audio-driven detection of moments of interaction}
\label{sec:moi}
Audio signals are particularly informative of moments of interaction. To complete day-to-day activities, we physically interact with objects in our environments. These interactions typically produce distinct audio patterns - short bursts of energy that span all frequencies.
This is illustrated in \figref{fig:intro}, where we visualize the untrimmed visual and audio data of a person performing a series of actions in the kitchen. The audio data is represented as a log mel spectrogram, where the x-axis represents time and y-axis the audio frequency in log-scale. As can be seen, moments of interaction appear in the spectrogram as \textit{vertical edges}, which can be easily detected. Once detected, short clips around the moments of interaction are collected into a dataset $\Dmoi$, and used for training.

% \todo{Let's see if we can defer some low-level info to implementation details.}
The remaining question is \textit{how to locate the timestamp of such vertical edges?} Intuitively, we do this by finding robust local maxima in the total energy (summed over all frequencies) of the spectrogram.
Concretely, let $M(t,\omega)$ be the value of the log mel spectrogram of an audio clip at time $t$ and frequency $\omega$. 
To remove the influence of background noise and overall audio intensity/volume, we compute the z-score normalization of the spectrogram for each frequency independently $\bar{M}(t,\omega)=\frac{s(t,\omega) - \mu_\omega}{\sigma_\omega + \epsilon}$, where $\epsilon$ is small constant for numerical stability. Here, $\mu_\omega$ and $\sigma_\omega$ are the mean and standard deviation of $M(t,\omega)$ over time, respectively.\footnote{Specifically, $\mu_\omega=\EV_t[M(t,\omega)]$, $\sigma_\omega^2=\EV_t[(M(t,\omega)-\mu_\omega)^2]$, and $\epsilon=1e-5$.}
% $\mu_\omega=\EV_t[s(t,\omega)]$ and $\sigma_\omega^2=\EV_t[(s(t,\omega)-\mu_\omega)^2]$ are the temporal mean and standard deviation of $s(t,\omega)$ over time, and $\epsilon=1e-5$ is a small constant for numerical stability. 
Next, we define moments of interaction as the set of timestamps which are local maxima of $\sum_\omega\bar{s}(t, \omega)$ (or peaks for short). Moreover, to avoid weak local maxima that may be caused by the noisy nature of audio signals, we ignore peaks with small prominence (lower than $1$)\footnote{The prominence of a peak is defined as the difference between the peak value and the minimum value in a small window around it.}. For further robustness, when multiple close peaks are found (less than $50$ms apart), only the highest prominence peak is kept. 
% Peak finding was conducted using python's scipy library~\cite{}.

% State change SSL
\subsection{Learning from audible state changes}
\label{sec:stc}
Physical interactions often cause both state changes in the environment and distinct audio signals. To leverage this natural co-occurrence, we propose a self-supervised task that seeks to \textit{associate the audio with changes in the visual state} during a moment of interaction.

% Leveraging cues from the audio spectrogram, we have now detected moments of interaction where object interactions and state changes are more likely to occur. These moments, thus, form a more informative dataset than the untrimmed and long-form videos. Over this dataset $\Dmoi$, we learn audio-visual representations using our proposed self-supervised task. The key idea being that \textit{audio representations should be associated with state changes} (as represented by changes in visual representations).

\begin{figure}
\centering
\begin{subfigure}{.53\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/system-stc.pdf}
  \caption{The proposed \loss formulation (\cref{sec:stc})}
  \label{fig:stc}
\end{subfigure}
\hfill%
\begin{subfigure}{.44\textwidth}
  \centering
  \includegraphics[width=\linewidth]{figures/system-avc.pdf}
  \caption{Audio-visual correspondence (\cref{sec:avc})}
  \label{fig:avc}
\end{subfigure}
\caption{\textbf{\method architecture for \loss and \avc tasks.} In both cases, short clips are extracted around moments of interaction~(MoI). (a). In \loss, the representation of a visual state change $\Delta \v_t$ is matched to the corresponding audio~$\a_t$. (b). \avc seeks to associate audio $a_t$ with the corresponding visual clips $v_t$.}
% , the visual representations themselves are matched to the corresponding audio.}
\label{fig:arch_heads}
\end{figure}

% In particular, over pairs in $\Dmoi$, we employ audio-visual correspondence learning (\cref{sec:avc}) to obtain representations that associate objects in the scene (visual feature) with their characteristic sound signatures (audio feature). Importantly, we hypothesize that correspondence alone is inefficient to learn representations that are informative of different object states and the transitions between states. To address this, we introduce an new self-supervised objective that seeks to associate sound with state changes as represented by changes in visual representations.

The proposed task is optimized by minimizing a loss with two negative log-likelihood terms to: (1) \textit{increase} the probability of associating the audio with the visual state change in the \textit{forward} (\ie correct) direction, (2) \textit{decrease} the probability of associating the audio with the visual state change in the \textit{backward} (\ie incorrect) direction. 
Consider, for example, the interaction of `closing a fridge door'. To optimize for this task, the audio of closing the door should be (1) similar to the visual transition \textit{opened door $\rightarrow$ closed door} and (2) dissimilar to the (backwards) transition \textit{closed $\rightarrow$ open}. This encourages learning of representations that are informative of object states, making them useful for a variety of egocentric tasks. Specifically, the audible state change (\loss) loss is defined as
% classification task, wherein the true directionality of the visual change (\ie, $\Delta \v_t$ or $-\Delta \v_t$) from the audio alone. 
% This is accomplished by minimizing the following binary cross-entropy loss
% \begin{equation}
% 	\Lastc = \EV_{v_t, a_t \in \Dmoi} \left[
% 	- \log \sigma\left(s_\Delta^+(v_t, a_t) / \tau\right)
% 	- \log \left( 1-\sigma\left(s_\Delta^-(v_t, a_t) / \tau\right)\right)\right]
% 	\label{eq:Lstc}
% \end{equation}
\begin{equation}
	\Lastc = \EV_{v_t, a_t \in \mathcal{D}_{\mathtt{MoI}}} \left[
	- \log \left(p^{\text{frwd}}(v_t, a_t)\right)
	- \log \left(1 - p^{\text{bkwd}}(v_t, a_t)\right)\right].
	\label{eq:Lstc}
\end{equation}
The probabilities ($p^{\text{frwd}}$, $p^{\text{bkwd}}$) are computed from cross-modal similarities
\begin{align}
p^{\text{frwd}}(v_t, a_t) &= \sigma\left(\mathtt{sim}\left(\Delta \v_t^{\text{frwd}}, \a_t\right)/ \tau\right),\\
p^{\text{bkwd}}(v_t, a_t) &= \sigma\left(\mathtt{sim}\left(\Delta \v_t^{\text{bkwd}}, \a_t\right)/\tau\right),
\end{align}
where $\tau=0.2$ is a temperature hyper-parameter, and $\sigma$ denotes the sigmoid function.
For better readability, we absorb the notations for the audio projection MLP head $h_A^{\loss}$ and the state change projection MLP head $h_{\Delta V}^{\loss}$ within $\mathtt{sim(\cdot, \cdot)}$, but their usage is clearly illustrated in \cref{fig:stc}. 
% Next, we detail the audio representations $\a_t$ and state change representations $\statechangef$ and $\statechangeb$.

\textbf{Audio representations ($\a_t$)} are obtained by encoding the trimmed audio clips $a_t$ via the audio encoder $f_A$ (shared across all objectives). 
As explained above, $\a_t$ is further projected via $h_A^{\loss}$ to a space where similarity to visual state changes is enforced.

% where $\sigma$ is a sigmoid function, and $\tau=0.2$ a temperature hyper-parameter. The positive and negative similarity scores ($s_\Delta^+$, $s_\Delta^-$) are computed as
% \begin{equation}
% s_\Delta^+(v_t, a_t) = \mathtt{sim}\left(h_{\Delta V}^{\loss}(\Delta \v_t); h_A^{\loss}(\a_t)\right)
% \quad\mbox{and}\quad
% s_\Delta^-(v_t, a_t) = \mathtt{sim}\left(h_{\Delta V}^{\loss}(-\Delta \v_t); h_A^{\loss}(\a_t)\right),
% \end{equation}
% where $h_{\Delta V}^{\loss}$ and $h_A^{\loss}$ are two multi-layer perceptrons that map $\Delta \v_t$ and $\a_t=f_A(a_t)$ into a common space (different from that used for audio-visual correspondence).

\textbf{State change representations ($\statechangef$, $\statechangeb$)} are computed by considering two non-overlapping visual clips for each moment of interaction $t$, at timestamps $t-\delta$ and $t+\delta$. 
The two clips, $v_{t-\delta}$ and $v_{t+\delta}$, are encoded via the visual encoder $f_V$ (shared across all tasks) and a projection MLP head $h_V^{\loss}$ (specific to the \loss task). Specifically, we represent forward and backward state changes as
\begin{align}
\statechangef &= h_V^{\loss} \circ f_V(v_{t+\delta}) - h_V^{\loss}\circ f_V(v_{t-\delta}),\\
\statechangeb &=h_V^{\loss} \circ f_V(v_{t-\delta})-h_V^{\loss}\circ f_V(v_{t+\delta}).
\end{align}

% The components necessary to compute these representations are: (1) a visual encoder $f_V$ that transforms the trimmed visual clip into visual features and (2) a projection MLP head $h_V^{\loss}$ that maps features.
% For each moment of interaction $t$, we consider two non-overlapping visual clips at timestamps $t-\delta$ and $t+\delta$, each of duration $2\delta$. Let these visual clips be called $v_{t-\delta}$ and $v_{t+\delta}$, respectively. 
% The representation of the two clips $\v_{t-\delta} = f_V(v_{t-\delta})$ and $\v_{t+\delta} = f_V(v_{t+\delta})$, is further transformed using a projection head dedicated to this loss ($h_V^{\loss}$).
% Quite symmetrically, we represent the state change as:
% \begin{align}
% \statechangef &= h_V^{\loss} \circ f_V(v_{t+\delta}) - h_V^{\loss}\circ f_V(v_{t-\delta})),\\
% \statechangeb &=h_V^{\loss} \circ f_V(v_{t-\delta}))-h_V^{\loss}\circ f_V(v_{t+\delta}),
% \end{align}
 
% This represents \textit{state change in the forward direction of time}

In summary, optimizing the loss of \cref{eq:Lstc} not only requires the audio representation $\a_t$ to be aligned with representation of the visual change $\statechangef$ that took place, but also to be different from the hypothetical backward state change $\statechangeb$. 

\subsection{Learning from audio-visual correspondences~\cite{de1994learning,arandjelovic2017look,morgado2021audio}}
\label{sec:avc}
Audio-visual correspondence (\avc) is a well-studied self-supervised methodology for learning unimodal audio and visual encoders. The key idea is to bring visual and audio clips into a common feature space, where the representations of audio-visual pairs are aligned. Note that \avc differs from the proposed \loss task, as \avc seeks to associate the audio $a_t$ with the corresponding visual clips $v_t$, as opposed to the change in visual state $\Delta \v_t$. As a result, visual representations learned through \avc are biased towards static concepts, while those learned through \loss are more sensitive to dynamic concepts. Since both types of representations can be useful for egocentric tasks, we further train the visual and audio encoders, $f_V$ and $f_A$, for the \avc task.

 Specifically, consider a dataset of audio-visual pairs $(v_i, a_i)$ with representations $\v_i=f_V(v_i)$ and $\a_i=f_A(a_i)$. In particular, we let $(v_i, a_i)$ be short clips extracted from sample $i$ around one of the detected moments of interest.
Then, following~\cite{morgado2021audio,cmc}, audio-visual correspondence is established by minimizing a cross-modal InfoNCE loss of the form
\begin{equation}
    \label{eq:avc}
	\Lavc = \EV_{v_i,a_i\sim{}\Dcal}\left[
	- \log \frac{e^{\s(\v_i, \a_i)/\tau}}{\sum_j e^{\s(\v_i, \a_j)/\tau}}
	- \log \frac{e^{\s(\v_i, \a_i)/\tau}}{\sum_j e^{\s(\v_j, \a_i)/\tau}}
	\right],
\end{equation}
where $\tau=0.07$ is a temperature hyper-parameter and $\texttt{sim}(\cdot, \cdot)$ denotes the cosine similarity.
Both terms in \cref{eq:avc} help bring $\v_i$ and $\a_i$ (\ie the positives) together. The key difference is whether the negative set is composed of audio representations $\a_j$ or visual representations $\v_j$ where $j \neq i$

For readability of \cref{eq:avc}, we once again absorb the notation for the audio and visual projection MLP heads ($h_A^\avc$ and $h_V^\avc$) within $\s(\cdot,\cdot)$, and illustrate their usage in \cref{fig:avc}.
\cref{fig:avc} also shows that we apply the \avc loss twice to associate both the visual clips (extracted slightly before and after the moment of interaction $t$) to the corresponding audio. 


% Both terms in \cref{eq:avc} help bring visual and audio representations \ie $\v_i$ and $\a_i$ (\ie the positives) closer. The key difference is what negatives are considered -- the first term operates on negative audio representations $\a_j$ and the second operates on negative visual representations $\v_j$, where $j \neq i$.
% Thus, minimizing \cref{eq:avc} ensures that corresponding audio and visual representations, $\a_i$ and $\v_i$, are closer to each other than to the representations of other negative samples ($\a_j$ and $\v_j$ for $j \neq i$), usually taken from the mini-batch under consideration.

% Egocentric datasets are often composed by long clips $(v, a)$ of duration $D$, which cannot be ingested in their entirety by the audio and visual models. Therefore, for efficient parallelization, models are often trained on short clips of duration $d<<D$. The standard solution is to \textit{randomly} sample moments in time $t\sim{}\mbox{Uniform}(0, D)$ around which to extract short clips for training.

\subsection{Training}
\label{sec:learning}
The audio-visual representation models $f_A$ and $f_V$ are trained to minimize both \avc and \loss losses
\begin{equation}
	\label{eq:loss_ssl}
	\Lcal = \alpha \Lavc + (1-\alpha) \Lastc
\end{equation}
where $\alpha$ is a weighting hyper-parameter between the two terms. While we experimented with different values of $\alpha$, we found that equal weighting produced best results.

\noindent\textbf{Implementation details}.
% In this work, we use a 3D CNN operating on short video clips as the visual encoder $f_V$ and a 2D CNN operating on mel spectrograms as the audio encoder $f_A$.
% In particular, we follow prior work on audio visual correspondence~\cite{morgado2021audio} and choose an R(2+1)D~\cite{r2p1d} of depth 18 and a 
We follow prior work on audio visual correspondence~\cite{morgado2021audio}, and use an R(2+1)D video encoder~\cite{r2p1d} with depth 18 and a 10-layer 2D CNN as the audio encoder. 
Two video clips are extracted around moments of interaction at a frame rate of 16 FPS each with a duration of $0.5$s, and separated by a gap of $0.2$s. 
Video clips are augmented by random resizing, cropping, and horizontal flipping resulting in clips of $8$ frames at a resolution of $112 \times112$,.
As for the audio, we extract clips of $2$s at $44.1$kHz and downsample them to $16$kHz. If the audio is stereo, we average the two waveforms to downgrade to mono,  and then convert the mono signal to a log mel spectrogram with $80$ frequency bands and $128$ temporal frames.
Models are trained with stochastic gradient descent for 100 epochs with a batch size of 128 trained over 4 GTX 1080 Ti GPUs, a learning rate of $0.005$ and a momentum of $0.9$. For Ego4D, we use a batch size of 512 trained over 8 RTX 2080 Ti GPUs with a learning rate of $0.05$. The two loss terms in \cref{eq:loss_ssl} are equally weighted with $\alpha=0.5$. 

% We implemented the cross-modal objective this way for computational reasons, \ie to avoid computing features for a third visual clip $v_t$. Despite lack of synchronization between the audio and visual clips, we did not find this to lead to worse representations since $\delta$ is set to a small enough value that audio visual correspondences are still meaningful.

% It should be noted that audio-visual correspondence is typically enforced between synchronized audio and visual clips~\cite{}. However, to compute $L_stc$, we need to sample two visual clips $v_{t-\delta}$ and $v_{t+\delta}$ and an audio clip $a_t$ around moment $t$. While the visual and audio clips are not perfectly aligned, $\delta$ is set to a small enough value that audio visual correspondences are still meaningful. Thus, we compute $\Lavc$ by averaging the audio-visual correspondences between the audio and both clips.


% Note that the loss $\Lcal_{SSL}$ operates on three clips $v^i_{t-\delta}$, $v^i_{t+\delta}$, $a^i_t$ extracted around moment $t$. The cross-modal loss $\Lcal_{\mbox{xCL}}$ is obtained as the average over two terms that seek to match the two visual clips $v^i_{t-\delta}$ and $v^i_{t+\delta}$ to audio $a^i_t$. We implemented the cross-modal objective this way for computational reasons,\ie to avoid computing features for a third visual clip $v_t^i$.


% \subsection{Implementation details}
% \paragraph{Models}

% \paragraph{Audio-visual data}


% \subsection{Model Input Definition}
% We consider a dataset of N samples $\mathcal{D} = \{d_i\}_{i=1}^{N}$ where each sample $d_i$ comprises an untrimmed video $d_i^v$ and its corresponding audio $d_i^a$. Using $d_i^a$, we generate a log spectrogram and find a set of $K$ peaks $\mathcal{P} = \{p^t\}_{t=1}^K$ where $p^t$ is a peak at time $t$ and is the local maxima for the amplitude within a local temporal neighborhood. We further define video clips to the left and right of peak $p^t$ as $v^{t_l}_i$ and $v^{t_r}_i$ respectively. We set the duration of each video clip to be $T$ seconds. We also consider a threshold $\delta$ on both sides of $p_t$ to denote the duration of peak. With this, we obtain $v^{t_l}_i$ and $v^{t_r}_i$ from timestamps $p_t - T - \delta$ to $p_t - \delta$ and $p_t + \delta$ to $p_t + \delta + T$ respectively. The time separation of $2\delta$ also allows $v^{t_l}_i$ and $v^{t_r}_i$ to not overlap each other.


% We try to learn the visual representation in a self-supervised manner from untrimmed videos by leveraging the audio modality in addition to the video modality.


% Given a dataset of N samples $D = {\{d_i}\}_{i=1}^{N}$ where each sample $d_i$ has a video $d_i^v$ and its corresponding audio $d_i^a$. For a sample, we generate a spectrogram using $d_i^a$ and find peaks in the audio signal. The peaks are defined as all the local maxima points by simply comparing the neighboring values. Let us denote a peak at time $t$ as $p_t$. Two video clips are taken from the left and right of the peak $p_t$ and denoted as $d_i^{v_l}$ and $d_i^{v_r}$. With respect to the peak $p_t$, $d_i^{v_l}$ is taken from $p_t - T - \delta$ to $p_t - \delta$ and $d_i^{v_r}$ is taken from $p_t + \delta$ to $p_t + T + \delta$. The $\delta$ parameter helps to avoid overlap between $d_i^{v_l}$ and $d_i^{v_r}$ clips and keep both the clips different. In parallel, the audio of both the $d_i^{v_l}$ and $d_i^{v_r}$ clips are taken together to have a final audio of duration $2*T$, denoted as $d_i^{a_{lr}}$.

% Once we have the above video and audio data, we process the data through a visual encoder $f_v$ and a audio encoder and $f_a$ to get the visual features for the left video clip as $v_l = f_v(d_i^{v_l})$, right video clip as $v_r = f_v(d_i^{v_r})$ and audio features as $a_{lr} = f_a(d_i^{a_{lr}})$ respectively. 

% \himangi{Should backbone and mlp be denoted differently?}

% \subsection{Losses}
% The visual features $v_l$, $v_r$ and ${a_{lr}}$ are finally used for the following loss functions - Contrastive Loss and Arrow of Time Order Loss.

% \textbf{Contrastive Loss}




% \textbf{Arrow of Time Order Loss :}  Using only the contrastive loss may not help in learning fine-grained action. The order loss is helpful in training the network to learn the order of the visual representations by leveraging the audio information. We consider the tuple with the order of $<v_l, a_{lr}, v_r>$ as the correct class having a label 1 and the the tuple with the incorrect order of $<v_r, a_{lr}, v_l>$ as the class having a label 0. An MLP is trained with the cross entropy loss for this binary classification task. With the application of this loss, the network learns the order of the left and right clip conditioned on the audio information.


==> latex/3-methods_moi_learning.tex <==
\section{Method}
We propose a method to learn audio-visual representations from untrimmed egocentric video data without relying on human annotations. The untrimmed nature of egocentric data poses major challenges for learning. For example, when there is little movement in the video, pace prediction objectives~\cite{} cannot be reliably predicted. Similarly, during moments of silence, the audio data cannot be reliably matched to the corresponding visuals in order to optimize audio-visual contrastive association objectives~\cite{}. These examples show that, when using untrimmed data, not all moments in time are useful for learning. In this work, we seek to identify useful moments in time, which we will call moments of interest (MoI).

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.8\linewidth]{figures/system.pdf}
    \caption{System. \label{fig:system}}
\end{figure}

\subsection{System}
Consider a large audio-visual dataset $\Dcal=\{(v_i, a_i)_{i=1}^N\}$ composed of $N$ untrimmed audio-visual pairs, where each sample $i$ is a long audio-visual stream with total duration $T_i$ seconds. 
Since the optimization of audio-visual models is typically conducted on short clips (sometimes as short as $0.5$s), most prior works randomly sample moments in time around which to extract training clips, $v_{it}$ and $a_{it}$~\cite{}.
Since, when learning from untrimmed data, a significant portion of the video may contain data with little value for training, we propose to screen each video for the most useful moments in time.
As illustrated in \cref{fig:system}, we screen each video using a model $f_{MoI}$ to score each moment $t$ according to the training value of clips centered around it. Then, the scores are used to guide the temporal sampling of clips used to train audio-visual representations, $f_A$ and $f_V$, through a pre-specified self-supervised objective $\Lcal_{SSL}$. The overall system can be trained by optimizing the following objective
\begin{eqnarray}
    \arg\min_{\theta_{MoI}, \theta_V, \theta_A} & \EV_{i\in\Dcal} \EV_{t\sim{}p^i_{MoI}} 
    \Lcal_{SSL}\left(f_A(a_{it};\theta_A), f_V(v_{it};\theta_V)\right) 
	\label{eq:ssl-opt1}\\
    \mbox{where} & p^i_{MoI} = \rho_t\left(f_{MoI}(a_{it}; \theta_{MoI}) / \tau \right)
    \label{eq:ssl-opt2}
\end{eqnarray}
$\rho_t$ is a softmax over time $t$, and $\tau$ a temperature coefficient that controls the peakiness of the predicted $p^i_{MoI}$ distribution.

Optimizing this objective introduces two major difficulties. First, the scoring function $f_{MoI}$ needs to be applied to every moment $t$ of each untrimmed sample in order to compute the full $P_{MoI}$ distribution. Thus, it is critical that $f_{MoI}$ is an high-throughput model. In this work, we experiment with small audio-driven models, and show that they are an excellent choice for this task, since audio can be indicative of many failure modes of SSL. Second, as is evident from \cref{fig:system}, $f_{MoI}$ cannot be directly optimized by back-propagating the loss gradients due to the non-differentiable temporal sampling and trimming operations. Instead, we optimize $f_{MoI}$ using policy gradients by thinking of it as a policy that simply selects the moments in time $t$ that lead to the lowest possible losses according to the current audio-visual models.

% \subsection{Predicting moments of interest}
% \textit{Spectrogram peaks?}
% Figure \todo{} illustrates a video clip with its corresponding audio of a person performing a series of actions in the kitchen. The audio is depicted as a log spectrogram where the color intensity denotes the amplitude. Brighter color intensity implies higher amplitude. We can observe in the figure that at the timestamp where an action starts or ends (such as opening or closing of the fridge), there is a sharp change in the amplitude. We can observe this change as a `vertical edge' on the log spectrogram. These edges form audio peaks that are local maxima in the amplitude. We extract these peaks and use them to split the untrimmed video into disjoint clips. We assume each obtained clip to exhibit a single action and uses these clips to learn in a self-supervised manner. 

% \textit{Audio model}

\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{figures/learning.pdf}
    \caption{Learning. \label{fig:learning}}
\end{figure}

\subsection{Learning}
We train the system by optimizing the loss of (\ref{eq:ssl-opt1}-\ref{eq:ssl-opt2}) over $\theta_{MoI}$, $\theta_{A}$ and $\theta_{V}$ in a alternating fashion. The optimization procedure can be decomposed into three steps, illustrated in \cref{fig:learning}.

\paragraph{Audio-driven MoI scoring} 
First, we use the current $f_{MoI}$ to compute an $MoI$ score for each moment in time $t\in[0,T]$, and convert the score into a sampling distribution
\begin{equation}
	\label{eq:moi}
	P^{k}_{MoI}(a_t) = \frac{\exp(f_{MoI}(a_t; \theta^{k}_{MoI})/\tau)}{\sum_k \exp(f_{MoI}(a_k; \theta^{k}_{MoI})/\tau)}.
\end{equation}
In practice, we sub-sample each sample and only evaluate $f_{MoI}$ every $0.5$s. We also restrict the softmax to a temporal window of $T=10$s. Since computing these distributions is computationally intensive, we recompute them sporadically throughout training (every few epochs of training). Section~\cref{exp:} explores the impact of the refresh frequency $P_{MoI}(a_t)$. 

The temperature hyper-parameter $\tau$ controls the exploration exploitation trade-off. High temperature values lead to sampling distributions $P_{MoI}$ that resemble a uniform distribution, while low temperature values lead to a peaky distribution with most mass concentrated around the time $t$ most likely to be a moment of interest, according to the current scoring function $f_{MoI}$. Since the scoring function is initially untrained, we begin training with a large value for $\tau_{\mbox{max}}$, thus promoting initial exploration of all moments in time. As training progresses and the scoring function $f_{MoI}$ becomes more accurate, we decrease $\tau$ down to a minimum value $\tau_{\mbox{min}}$ using a half-cosine schedule~\cite{}.


\paragraph{Audio-visual representation learning}
Next, for each video, we extract audio-visual clips, $a_t$ and $v_t$, centered around moments of interest $t$ sampled from the pre-computed sampling distributions $P_{MoI}$. These audio-visual clips are used to train the audio and visual encoders, $f_A$ and $f_V$, by optimizing the pre-defined self-supervised loss $\Lcal_{SSL}$. This is equivalent to optimize (\ref{eq:ssl-opt1}-\ref{eq:ssl-opt2}), given the current MoI scoring model $f^{k}_{MoI}$.
\begin{equation}
	\label{eq:ssl}
	\theta_A^{k+1}, \theta_V^{k+1} = 
	\arg\min_{\theta_V, \theta_A} \EV_{i\in\Dcal} \EV_{t\sim{}P^{k}_{MoI}} 
    \Lcal_{SSL}\left(f_A(a_{it};\theta_A), f_V(v_{it};\theta_V)\right) 
\end{equation}
Since as the sampling distribution $P^{k}_{MoI}$ changes, the optimal audio-visual encoders should also change, we do not optimize \cref{eq:av-ssl} until convergence. Instead, we train the encoders $f_A$ and $f_V$ for a fixed number of epochs, $N_{SSL}$, before switching to the MoI regression phase.


\paragraph{MoI regression}
Given the current audio-visual models, $f_A^{k+1}$ and $f_V^{k+1}$, we train the MoI scoring function $f_{MoI}$ to optimize the loss of (\ref{eq:ssl-opt1}-\ref{eq:ssl-opt2}). Since the sampling and clipping operations are non-differentiable, we optimize $f_{MoI}$ using policy gradients~\cite{} to maximize the following rewards
\begin{equation}
	\label{eq:reward}
	r_{it} = -\Lcal_{SSL}\left(f_A(a_{it};\theta_A^{k+1}), f_V(v_{it};\theta_V^{k+1})\right)
\end{equation}
Specifically, at each step, we sample a batch of untrimmed videos, and trim them into audio-visual clips $a_{it}$ and $v_{it}$ by sampling from $P^{k}_{MoI}(a_i)$. The clips are then fed to the audio visual models to compute the rewards. Finally, the $f_{MoI}$ model is optimized by taking a step into the policy gradient direction~\cite{} given by
\begin{equation}
	\label{eq:policy_grad}
	\nabla_{\theta_{MoI}} \Lcal_{SSL}({\theta_{MoI}}) \propto \EV_{i\in\Dcal, t\sim{}P^{k}_{MoI}}\left[ G_{it} \nabla_{\theta_{MoI}} \log P_{MoI}(a_t; \theta_{MoI}) \right]
\end{equation}
where $P_{MoI}$ is the policy function of \cref{eq:moi}, $G_{it} = (r_{it} - \mu_r) / \sigma_r$ is a normalized reward, and $\mu_r$ and $\sigma_r$ are the mean and standard deviations of recent scores computed by exponential moving average with coefficient $m=0.9$.
We highlight that the policy gradient of \cref{eq:policy_grad} provides an intuitive update rule for the MoI scoring function, since $f_{MoI}$ is optimized to increase the scores for moments in time with rewards $r_{it}$ higher than average $\mu_r$, and lower the MoI scores of moments with $r_{it}$ lower than $\mu_r$. As a result, as training progresses, $f_{MoI}$ should get better at predicting the moments in time that for which $\Lcal_{SSL}$ can be optimized.


\subsection{Self-supervised learning}
\label{sec:ssl}
In this work, we seek to learn visual representations from audio-visual data.
While the proposed framework can easily generalize to any loss or combination of losses, we focus on audio-visual representation learning. We experimented with a combination of two loss terms, previously introduced in prior work: audio-visual instance discrimination~\cite{} and clip order prediction~\cite{}.


\paragraph{Audio-visual instance discrimination.}
Audio-visual instance discrimination has been extensively studied in prior work~\cite{}, and has been shown to yield strong video representations for tasks like action recognition~\cite{}. In its simplest form, given a batch of audio-visual clips $\Bcal=\{(v_i, a_i)_{i=1}^B\}$, audio-visual instance discrimination seeks to optimize the sample loss of the form
\begin{equation}
	\Lcal_{xID}(v_i, a_i) = 
	- \log \frac{\exp(s(z_i^v, z_i^a)/\tau)}{\sum_j \exp(s(z_i^v, z_j^a)/\tau)}
	- \log \frac{\exp(s(z_i^a, z_i^v)/\tau)}{\sum_j \exp(s(z_i^a, z_j^v)/\tau)}
\end{equation}
where $s(z_1, z_2)=\frac{z_1^Tz_2}{\|z_1\|\|z_2\|}$ denotes the cosine similarity, $\tau$ a temperature hyper-parameter, and $z_i^a=f_A(a_i)$ and $z_i^v=f_V(v_i)$ are the audio and visual representations.

\paragraph{Audio conditioned clip order prediction.}
Order prediction objectives have also been studied in prior work~\cite{}. They have also been shown to produce strong video representations~\cite{} and to be complementary to audio-visual instance discrimination~\cite{}. In its simplest form, order prediction is conducted from visual data alone. Let $v^i_{t-\delta}$ and $v^i_{t+\delta}$ be two clips taken from the same video $v^i$ at times $t-\delta$ and $t+\delta$ where $2\delta$ denotes a temporal distance between the two clips. Video-based order prediction is accomplished through a prediction head $g_{vOP}$ learned to optimize
\begin{equation}
	\Lcal_{vOP}(v^i_{t-\delta}, v^i_{t+\delta}) = \log\left( 1+ \frac{\exp(g_{vOP}(v^i_{t+\delta}, v^i_{t-\delta}))}{\exp(g_{vOP}(v^i_{t-\delta}, v^i_{t+\delta}))}\right)
\end{equation}
where $g_{vOP}(v^i_{t+\delta}, v^i_{t-\delta})$ is implemented by concatenating the two input features and feeding it to a multi-layer perceptron with a singe output.
This objective creates embeddings that are sensitive to the arrow of time in videos, since $g_{vOP}(v_{t_1}, v_{t_2})$ is trained to output large values only if $t_1>t_2$. This sensitivity promotes better temporal understanding, which leads to good representations for actions. 

However, we argue that often temporal order prediction is under-specified. For example, consider the case of two visual clips, one where someone is holding a pan and another where the pan is on a stove. Predicting the correct order depends on whether the video was depicting someone placing the pan on the stove or someone removing it from the stove. Without access to additional information, predicting the correct order cannot be done. 
To address this problem, we enhance clip order objectives by conditioning the prediction on audio data. In the previous example, the audio can completely disambiguate which action was taking place, as setting the pan on the stove would likely produce a contact sound. A specific action can be better understood through the unique audio associated with every action. Specifically, we can instead train the models to minimize the following audio-visual order prediction objective
\begin{equation}
	\Lcal_{avOP}(v^i_{t-\delta}, v^i_{t+\delta}, a^i_t) = \log\left( 1+ \frac{\exp(g_{vOP}(v^i_{t+\delta}, v^i_{t-\delta}, a^i_t))}{\exp(g_{vOP}(v^i_{t-\delta}, v^i_{t+\delta}, a^i_t))}\right)
\end{equation}

\paragraph{Combined objective.}
Above, we introduced two self-supervised objectives. We combined them using a multi-task loss of the form.
\begin{equation}
	\label{eq:loss_ssl}
	\Lcal_{SSL}(v^i_{t-\delta}, v^i_{t+\delta}, a^i_t) = 
	\alpha_1 \frac{\Lcal_{\mbox{xCL}}(v^i_{t-\delta}, a^i_t) + \Lcal_{\mbox{xCL}}(v^i_{t+\delta}, a^i_t)}{2} + 
	\alpha_2 \Lcal_{\mbox{avOP}}(v^i_{t-\delta}, v^i_{t+\delta}, a^i_t)
\end{equation}
where $\alpha_1$ and $\alpha_2$ are weighting hyper-parameters. Note that the loss $\Lcal_{SSL}$ operates on three clips $v^i_{t-\delta}$, $v^i_{t+\delta}$, $a^i_t$ extracted around moment $t$. The cross-modal loss $\Lcal_{\mbox{xCL}}$ is obtained as the average over two terms that seek to match the two visual clips $v^i_{t-\delta}$ and $v^i_{t+\delta}$ to audio $a^i_t$. We implemented the cross-modal objective this way for computational reasons,\ie to avoid computing features for a third visual clip $v_t^i$.


\subsection{Implementation details}
\paragraph{Models}

\paragraph{Audio-visual data}


\subsection{Model Input Definition}
We consider a dataset of N samples $\mathcal{D} = \{d_i\}_{i=1}^{N}$ where each sample $d_i$ comprises an untrimmed video $d_i^v$ and its corresponding audio $d_i^a$. Using $d_i^a$, we generate a log spectrogram and find a set of $K$ peaks $\mathcal{P} = \{p^t\}_{t=1}^K$ where $p^t$ is a peak at time $t$ and is the local maxima for the amplitude within a local temporal neighborhood. We further define video clips to the left and right of peak $p^t$ as $v^{t_l}_i$ and $v^{t_r}_i$ respectively. We set the duration of each video clip to be $T$ seconds. We also consider a threshold $\delta$ on both sides of $p_t$ to denote the duration of peak. With this, we obtain $v^{t_l}_i$ and $v^{t_r}_i$ from timestamps $p_t - T - \delta$ to $p_t - \delta$ and $p_t + \delta$ to $p_t + \delta + T$ respectively. The time separation of $2\delta$ also allows $v^{t_l}_i$ and $v^{t_r}_i$ to not overlap each other.


We try to learn the visual representation in a self-supervised manner from untrimmed videos by leveraging the audio modality in addition to the video modality.


Given a dataset of N samples $D = {\{d_i}\}_{i=1}^{N}$ where each sample $d_i$ has a video $d_i^v$ and its corresponding audio $d_i^a$. For a sample, we generate a spectrogram using $d_i^a$ and find peaks in the audio signal. The peaks are defined as all the local maxima points by simply comparing the neighboring values. Let us denote a peak at time $t$ as $p_t$. Two video clips are taken from the left and right of the peak $p_t$ and denoted as $d_i^{v_l}$ and $d_i^{v_r}$. With respect to the peak $p_t$, $d_i^{v_l}$ is taken from $p_t - T - \delta$ to $p_t - \delta$ and $d_i^{v_r}$ is taken from $p_t + \delta$ to $p_t + T + \delta$. The $\delta$ parameter helps to avoid overlap between $d_i^{v_l}$ and $d_i^{v_r}$ clips and keep both the clips different. In parallel, the audio of both the $d_i^{v_l}$ and $d_i^{v_r}$ clips are taken together to have a final audio of duration $2*T$, denoted as $d_i^{a_{lr}}$.

Once we have the above video and audio data, we process the data through a visual encoder $f_v$ and a audio encoder and $f_a$ to get the visual features for the left video clip as $v_l = f_v(d_i^{v_l})$, right video clip as $v_r = f_v(d_i^{v_r})$ and audio features as $a_{lr} = f_a(d_i^{a_{lr}})$ respectively. \himangi{Should backbone and mlp be denoted differently?}

\subsection{Losses}
The visual features $v_l$, $v_r$ and ${a_{lr}}$ are finally used for the following loss functions - Contrastive Loss and Arrow of Time Order Loss.

\textbf{Contrastive Loss}




\textbf{Arrow of Time Order Loss :}  Using only the contrastive loss may not help in learning fine-grained action. The order loss is helpful in training the network to learn the order of the visual representations by leveraging the audio information. We consider the tuple with the order of $<v_l, a_{lr}, v_r>$ as the correct class having a label 1 and the the tuple with the incorrect order of $<v_r, a_{lr}, v_l>$ as the class having a label 0. An MLP is trained with the cross entropy loss for this binary classification task. With the application of this loss, the network learns the order of the left and right clip conditioned on the audio information.




==> latex/4-experiments.tex <==
\section{Experiments}
In this section, we demonstrate the benefits of identifying moments of interaction and learning state-aware representations through an audible state-change objective. We also show that, while large scale audio-visual correspondence (\avc) is beneficial, it is not sufficient to learn state-aware representations required for egocentric tasks. The setup used for our experiments is described in \cref{sec:setup}. Results and discussion of main takeaways are presented in \cref{sec:results}.

\subsection{Experimental Setup}
\label{sec:setup}
\textbf{Datasets}. We evaluate on two egocentric datasets: \epickitchens~\cite{damen2020rescaling} and Ego4D~\cite{grauman2021ego4d}. \epickitchens contains 100 hours of activities in the kitchen.
Ego4D contains 3670 hours of egocentric video covering daily activities in the home, workplace, social settings, \etc. For experiments on Ego4D, we use all videos from the Forecasting and Hand-Object interaction subsets.

% \textbf{Downstream Tasks and Metrics}
% We evaluate the efficiency of the visual representations learned by our model on the following downstream tasks: \textbf{(1). Action Recognition (AR):} Given a short video clip, the network tries to classify the verb and noun associated with this clip. We use both the EPIC-KITCHENS-100 and Ego4D datasets for evaluating on this task and report the top-1 and top-5 accuracy (\%) for both verb and noun in Table~\ref{tbl:ek100main}. \textbf{(2). Object state change classification (StCC)} For a short video clip, the network tries to classify if an object state undergoes a change or not. We use Ego4D for this downstream task and report the State Change Classification Accuracy~(\%) in Table~\ref{tbl:ego4dmain}.  \textbf{(3). Long-term action anticipation (LTA)} The network tries to predict the camera wearer's future sequence of actions. For this task as well, we use the Ego4D dataset and report the edit distance metric, ED@(Z=20)~\cite{grauman2021ego4d}. This metric quantifies the dissimilarity between the prediction and ground truth by counting the minimum number of operations required to convert the prediction to ground truth. The operations include insertions, deletions, substitutions and transpositions. Z refers to the number of actions predicted at a timestamp.  
% \textbf{(3). Point-of-no-return temporal localization} For a short video clip of a state change, the network tries to predict the keyframe that indicates point-of-no-return, that is, the timestamp at which the state change begins.

\textbf{Baselines and ablations.}
We consider various baselines as well as ablated versions of \method. \textit{Random} represents an untrained (randomly initialized) model and \textit{AVID}~\cite{morgado2021audio} is a state-of-the-art model pre-trained on 2M audio-visual pairs from AudioSet~\cite{gemmeke2017audio} with only audio-visual correspondence.
For the full method \textit{\method}, we initialize the model weights from AVID before training on moments of interaction to minimize both \avc and state change loss, \loss. We also evaluate our method trained without AVID initialization (\textit{\method from scratch}), trained with only \avc (\textit{\method w/o \loss}), only state change losses (\textit{\method w/o \avc}), and trained on random moments in time (\textit{\method w/o MoI}). Finally, we compare our approach with the fully supervised methods presented in Ego4D~\cite{grauman2021ego4d}.

\textbf{Downstream tasks.}
After self-supervised pre-training, the models are evaluated on a range of egocentric downstream tasks. This is done, as is standard, by appending a task specific decoder to the backbone model, and training the decoder on a small annotated dataset. The tasks are:
% \begin{itemize}[leftmargin=10pt]\compresslist
\begin{itemize}[leftmargin=20pt]
    \item \emph{Video action recognition~(AR) on \epickitchens and Ego4D.} Given a short video clip, the task is to classify the `verb' and `noun' of the action taking place. This is done using two separate linear classifiers trained for this task. We report the top-1 and top-5 accuracies, following~\cite{damen2020rescaling} (\cref{tbl:ek100main}) and \cite{grauman2021ego4d} (\cref{tbl:ego4dmain}). We also evaluate on the unseen participants, head classes, and tail classes of \epickitchens in \cref{tbl:ek100unseenheadtail}. Through this task, we assess the efficacy of the spatial-temporal representations learned by the model in differentiating among different verbs and nouns. 
    \item \emph{Long-term action anticipation~(LTA) on Ego4D.} Given a video, the task is to predict the camera wearer's future sequence of actions. For this task, the model is first presented with 4 consecutive clips of $2$s, which are encoded using our visual backbone $f_V$. Following~\cite{grauman2021ego4d}, the representations are concatenated and fed to 20 separate linear classification heads to predict the following 20 actions.
    Performance is measured using the edit distance metric ED@(Z=20)~\cite{grauman2021ego4d}.\footnote{Edit distance measures the minimum number of operations required to convert the predicted sequence of actions to ground truth. To account for multi-modality of future actions, it also allows the model to make $Z=20$ predictions, and only accounts for the best prediction.} With the help of this task, we can evaluate if the representations learned by the model can be employed for long-horizon planning where the actions can change and may be of arbitrary duration.  Results are reported in \cref{tbl:ego4dmain}. 
    \item \emph{State change classification~(StCC) on Ego4D.} Given a video clip, the task is to classify if an object undergoes a state change or not. The video clip is encoded by $f_V$ and a state change classification head is used which performs global average pooling on the entire feature tensor and is followed by a classification layer. Performance is measured through the State Change Classification Accuracy~(\%), and reported in \cref{tbl:ego4dmain}. This task is ideal for assessing the ability of the model in understanding the temporal change happening in the state of an object.
    \end{itemize}

\subsection{Discussion of results}
\label{sec:results}
\input{tables/ek100_main}
\input{tables/ego4d_main}
\input{tables/unseen_head_tail}

As can be seen in \cref{tbl:ek100main} and \cref{tbl:ego4dmain}, \method outperforms all other methods across all downstream tasks. Overall, this can be attributed to its ability to focus on interactions, both by detecting when they occur and by learning representations that are sensitive to interactions. A closer analysis of these results reveals several insights that we discuss next.
% \textbf{EPIC-KITCHENS-100: } In terms of verb top-1 accuracy, an improvement of of 5.09\% compared to AVID Weights~\cite{morgado2021audio} and a 3\% compared to \textit{\method w/o MoI Sampling} is observed. Whereas, in terms of noun top-1 accuracy, an improvement of 2.25\% compared to AVID Weights, and 2.92\% compared to \textit{\method w/o MoISampling} is observed. We also report the results over the unseen participants, head classes, and tail classes. <observation> \textbf{Ego4D: } For e

% \vspace{-0.5em}
\paragraph{\method enhances large-scale \avc driven approaches.}
Prior work on self-supervised audio-visual learning has shown strong audio-visual representations for action recognition~\cite{morgado2021audio, morgado2021robust}. One question that we seek to answer is, how useful these are representations to egocentric tasks and what are their limitations? To answer this question, we compare our model trained from scratch, \textit{\method~(Scratch)}, with our model using the weights from AVID~\cite{morgado2021audio} as initialization for both the visual and audio encoders. We also compare our method to standalone AVID \ie without further self-supervised training. 
Comparing rows (2) and (7) in \cref{tbl:ek100main} and \cref{tbl:ego4dmain}, it is clear that \method enhances large-scale \avc pre-training by significant margins, leading to absolute improvements of $5\%$ in top-1 verb accuracy on \epickitchens, $4.2\%$ on Ego4D, $5.2\%$ increase in state-change classification accuracy, and $5.6\%$ reduction on the edit distance for long-term anticipation.
Comparing rows (6) and (7), we also see that large-scale AVID pre-training enhances the representations learned by \method on \epickitchens significantly but only marginally on Ego-4D. This is likely due to the significantly large diversity of scenes in Ego4D. Thus, while relying on large-scale audio-visual pre-training (as with AVID) can help avoid overfitting on smaller egocentric datasets, this is less critical when training on larger and more diverse data.

% \vspace{-0.5em}
\paragraph{Detecting moments of interaction (MoI) helps representation learning.}
We hypothesize that to learn good representations for egocentric data of daily activities, self-supervised learning should focus on moments in time when interactions occur. To assess whether our audio-driven MoI detection algorithm helps representation learning, we compare \textit{\method} with an ablated version, \textit{\method w/o MoI}, where the model is trained on audio-visual clips extracted at \textit{random} from the untrimmed videos.
As can be seen by comparing rows (5) and (7) in \cref{tbl:ek100main} and \cref{tbl:ego4dmain}, sampling clips around MoI leads to significantly better representations for all egocentric downstream tasks that we study. 
% By having an explicit state change objective function and the moments of interactions which are likely to be aligned with the actual state changes, our model gains a better understanding of how the state changes by an interaction and how the actions transition over time. 
% This allows \textit{\method} to perform better than \textit{\method w/o MoI}. 
Moreover, even though \textit{\method w/o MoI} trains with \loss, it is unable to fully leverage the state change objective function without the information of moments of interactions which leads to a worse performance. 
This suggests that, an explicit state change objective function and sampling video clips around moments of interactions (which are likely to be aligned with the actual state changes) together provide an information-rich feedback to our model in better understanding how the state changes by an interaction and how the actions transition over time.
These results also clearly show that the proposed MoI detection procedure is able to find moments in time that are especially useful for learning representations of daily activities. We emphasize the simplicity and effectiveness of our audio-driven detector, which shows how informative audio can be when searching for moments of interaction. In the future, we believe that learning-based approaches could further enhance MoI detection, and further improve the learned audio-visual representations. We also show several qualitative examples of detected MoI in the supplement.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/tsne_uj_3.pdf}
    \vspace{-5mm}
    \caption{t-SNE visualization of the feature representations learned by \textit{\method} and \textit{AVID} for a video consisting of fine-grained actions over time. For a simpler visualization, we consider all the videos belonging to a single participant. A larger spread in the t-SNE of \textit{\method} indicates more distinct state-aware representations.}
    \label{fig:tsne}
    \vspace{-2mm}
\end{figure}

% \vspace{-0.5em}
\paragraph{\avc and \loss are complementary.}
To assess the impact of both terms in \cref{eq:loss_ssl}, we evaluate \textit{\method} trained without $\Lavc$ and without $\Lastc$.
Comparing rows (3), (4) to row (2) in \cref{tbl:ek100main} and \cref{tbl:ego4dmain} shows that each term enhances the representations obtained through large-scale audio-visual pre-training (AVID). Furthermore, comparing the ablated models in rows (3) and (4) to the full model in row (7) shows that these two terms are complementary to each other. This is because the \avc and \loss tasks encourage learning of representations with different characteristics. \avc focuses on learning visual representations that are informative of what kind of sounding objects are present in the video, while \loss forces the model to differentiate between visual representations that occur before and after state change interactions.

% \vspace{-0.5em}
\paragraph{\method encourages state-aware representation learning.}
To study the representations learned by our approach for different states, we generate a t-SNE plot~\cite{tsne} for \textit{\method} and \textit{AVID} as shown in~\cref{fig:tsne}. For generating a simpler visualization, a small dataset is prepared consisting of all the videos corresponding to a single participant, \textit{P01}, in \epickitchens and split into clips of $0.5$s. We can observe that there is a larger spread in the t-SNE plot for \textit{\method} than \textit{AVID}. A larger spread indicates that the representations of the various states are significantly different from each other and form more distant clusters as shown by \textit{\method}. Whereas, if the state representations are similar to each other, they are clustered together and show lesser spread as shown by \textit{AVID}. MoI are the key moments of interactions with an object in an environment where the state is changing. \textit{AVID} has no such information about the key moments and also does not have an explicit state change objective function. Therefore, it is unable to discriminate between the \textit{before} and \textit{after} state of an action and has less effective state-aware information in its representations.

\vspace{-1em}
\paragraph{\method representation are more generalizable and robust to long-tail.}
% \paragraph{Generalization ability and robustness of \method representations}
To assess \method in a scenario with domain shift, we evaluate on unseen participants that were fully excluded from the pre-training of \method. \cref{tbl:ek100unseenheadtail} shows that \method significantly outperforms baselines and ablations, indicating that representation learning by our model provides much better generalization. Moreover, the verb and noun classes in EPIC-Kitchens-100 exhibit a long-tailed distribution. When further compared on head and tail classes separately in \cref{tbl:ek100unseenheadtail}, we can observe that \method outperforms all other methods highlighting its higher robustness on a long-tailed distribution.

% In \cref{tbl:ek100unseenheadtail}, unseen participants consist of the subjects that were excluded from the training of \textit{\method} and are only used for evaluation. A better performance of \textit{\method} compared to the baselines and ablations indicates that the representations learned by the model are robust to the domain shift. It is able to perform well even on the subjects that are unseen during the model training. Additionally, the verb and noun classes in the \epickitchens dataset are long-tail distributed. Our model also outperforms baselines on both head and tail classes.

\vspace{-0.8em}
\paragraph{Self-supervised vs supervised representation learning}
\cref{tbl:ego4dmain} also compares \method to fully supervised methods introduced in Ego4D~\cite{grauman2021ego4d} (rows S1, S2 and S3).
We can observe that \method can also perform competitively to the fully supervised approaches when we have access to larger and more diverse data.
% \method can mostly bridge the gap to the fully supervised  supervised approaches, leaving only a small gap. 
With further focus on SSL for untrimmed datasets, SSL methods will be able to match supervised approaches, and our work takes a step towards it.

% Moved to supplementary
% \input{tables/unseen_head_tail}



==> latex/5-conclusions.tex <==
\section{Conclusion}
In this work, we propose an audio-driven self-supervised method for learning representations of egocentric video of daily activities. We show that in order to learn strong representations for this domain, two important challenges need to be addressed.
First, learning should focus on moments of interaction (MoI). Since these moments only occur sporadically in untrimmed video data, we show that MoI detection is an important component of representation learning in untrimmed datasets.
Second, learning should focus on the consequences of interactions, \ie, changes in the state of an environment caused by agents interacting with the world. In particular, by seeking to identify visible state changes from the audio alone, we can learn representations that are potentially more aware of the state of the environment and hence, particularly useful for egocentric downstream tasks.

==> neurips/99_checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
% %   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
% %   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{We point out in Section 4.2: Discussion of results, the potential avenues for future research inspired by the limitations of our method.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Refer to the Supplement Material}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{The code and instructions are given in the supplemental material. However, the dataset is too large for the supplement material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Refer to Section 3.5: Implementation Details}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{Since the train and test set are too large, it takes a lot of time and resource to run the experiments multiple times. However, errors bars are expected to be small, given their sizes.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Refer to Section 3.5: Implementation Details}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> tables/ego4d_ablation.tex <==
\begin{table}[]
\centering
\begin{tabular}{l|c|c|c|c}
                                      & \textbf{State Change Classification accuracy (\%)} & \textbf{Task 2} & \textbf{Task 3} & \textbf{Task 4} \\ \hline
\textbf{SSRL w/o CLR Loss}            &                                                    &                 &                 &                 \\
\textbf{SSRL w/o State Change Loss}   &                                                    &                 &                 &                 \\
\textbf{SSRL w/o AVID initialization} &                                                    &                 &                 &                 \\
\hline
\textbf{SSRL w/ spectrogram peaks}                         &                                                    &                 &                 &                \\
\hline
\end{tabular}
% \vspace{0.5em}
\caption{}
\label{tbl:ego4dablation}
\end{table}

==> tables/ego4d_main.tex <==
% \begin{table}[]
% \centering
% \begin{tabular}{l|c|c|c|c}
%                                      & \textbf{State Change Classification accuracy (\%)} & \textbf{Task 2} & \textbf{Task 3} & \textbf{Task 4} \\ \hline
% \textbf{Scratch (Random weights)}    &        -                                            &         -        &    -             &        -         \\
% \textbf{AVID}                        &                                                    &                 &                 &                 \\
% \textbf{SSRL w/ random peaks}      &                                                    &                 &                 &                 \\
% \hline
% \textbf{SSRL w/ spectrogram peaks} &                                                    &                 &                 &           \\
% \hline
% \end{tabular}
% \vspace{0.5em}
% \caption{}
% \label{tbl:ego4dmain}
% \end{table}

% \begin{table}[]
% \begin{tabular}{ccccc||cccc}
% \textbf{AVID} & \textbf{CLR Loss} & \textbf{StC Loss} & \textbf{Random Peaks} & \textbf{Spectrogram Peaks} & \textbf{Verb1} & \textbf{Noun1} & \textbf{Verb5} & \textbf{Noun5} \\ \hline
% -             &                   &                   &                       &                            & -              &                &                &                \\
%               & -                 &                   &                       &                            &                &                & -              &                \\
%               &                   & -                 &                       &                            &                & -              &                &                \\
%               &                   &                   & -                     &                            &                &                &                & -              \\
%               &                   &                   &                       & -                          &                &                &                &    \\
% \hline
% \end{tabular}
% \vspace{0.5em}
% \caption{}
% \label{tbl:ego4dmain}
% \end{table}

% \begin{table}[h]
% \begin{tabular}{cccp{15mm}p{18mm}||p{15mm}ccc}
% \textbf{AVID~\cite{morgado2021audio}} & \textbf{CLR Loss} & \textbf{StC Loss} & \textbf{Random \newline Peaks} & \textbf{Spectrogram \newline Peaks} & \textbf{State Change \newline Classification Accuracy (\%)} & \textbf{Task 2} & \textbf{Task 3} & \textbf{Task 4} \\ \hline
%  \checkmark           &      \checkmark             &                   &                       &            \checkmark                &    63.60           &                &                &                \\
%  \checkmark             &                  &    \checkmark               &                       &  \checkmark                          &    64.00            &                &               &                \\
%               &    \checkmark               & \checkmark                &                       &     \checkmark                       &          66.20       &              &                &                \\
%               &                  &                   &                      &                           &    51.80            &               &                &               \\
% \checkmark          &                   &                   &                       &                  &     61.11           &                &                &              \\
% \checkmark          &   \checkmark                &                   &     \checkmark                 &                          &                &                &                &              \\
% \checkmark          &   \checkmark                &     \checkmark              &     \checkmark                 &                          &     62.90           &                &                &              \\
% \hline
% \checkmark          &   \checkmark                &     \checkmark              &                      &       \checkmark                   &    \textbf{66.30}            &                &                &              \\
% \hline
% \end{tabular}
% \vspace{0.5em}
% \caption{Downstream Tasks on Ego4D}
% \label{tbl:ego4dmain}
% \end{table}

\begin{table}[t]
\centering
\resizebox{0.99\textwidth}{!}{
\begin{tabular}{|l|cccc|c|cc|cc|}
\multicolumn{5}{c}{} & \multicolumn{1}{c}{\bf StCC} & \multicolumn{2}{c}{\bf AR } & \multicolumn{2}{c}{\bf LTA} \\ \hline
\multirow{2}{*}{\textbf{Method}} & 
\multirow{2}{*}{\textbf{$\Lavc$}} & 
\multirow{2}{*}{\textbf{$\Lastc$}} & 
\multirow{2}{*}{\textbf{MoI}} &
\multirow{2}{*}{\thead{\textbf{AVID}\\\textbf{Init}~\cite{morgado2021audio}}} & 
\multirow{2}{*}{\textbf{Acc} $\uparrow$} &
\multicolumn{2}{c|}{\textbf{Top1 Acc} $\uparrow$} &
\multicolumn{2}{c|}{\textbf{ED@(Z=20)} $\downarrow$} \\
&&&&&& Verb & Noun & Verb & Noun \\\hline
\textcolor{lightgray}{(S1) I3D-ResNet-50~\cite{carreira2017quo, grauman2021ego4d}} & \textcolor{lightgray}{NA} & \textcolor{lightgray}{NA} & \textcolor{lightgray}{NA} & \textcolor{lightgray}{NA} & \textcolor{lightgray}{68.70} & \textcolor{lightgray}{-} & \textcolor{lightgray}{-} & \textcolor{lightgray}{-} & \textcolor{lightgray}{-} \\
\textcolor{lightgray}{(S2) SlowFast~\cite{feichtenhofer2019slowfast, grauman2021ego4d}} & \textcolor{lightgray}{NA} & \textcolor{lightgray}{NA} & \textcolor{lightgray}{NA} & \textcolor{lightgray}{NA} & \textcolor{lightgray}{-} & \textcolor{lightgray}{-} & \textcolor{lightgray}{-} & \textcolor{lightgray}{0.747} & \textcolor{lightgray}{0.808} \\
\textcolor{lightgray}{(S3) MViT~\cite{fan2021multiscale, grauman2021ego4d}} & \textcolor{lightgray}{NA} & \textcolor{lightgray}{NA} & \textcolor{lightgray}{NA} & \textcolor{lightgray}{NA} & \textcolor{lightgray}{-} & \textcolor{lightgray}{-} & \textcolor{lightgray}{-} & \textcolor{lightgray}{0.707} & \textcolor{lightgray}{0.901} \\
\hline
(1) Random        & & & &   						       & 51.80 & 17.4 & 7.7 & 0.831 & 0.936 \\
(2) AVID~\cite{morgado2021audio}          & & & & \checkmark  					   & 61.11 & 18.3 & 10.7 & 0.811 & 0.919 \\
(3) \method w/o \avc          & & \checkmark & \checkmark & \checkmark & 64.00 & 20.3 & 12.4 & 0.781 & 0.854 \\
(4) \method w/o \loss          & \checkmark & & \checkmark & \checkmark & 63.60 & 21.1 & 13.5 & 0.774 & 0.853 \\
(5) \method w/o MoI & \checkmark & \checkmark & & \checkmark & 62.90 & 19.8 & 11.2 & 0.792 & 0.868 \\
(6) \method (scratch)     & \checkmark & \checkmark & \checkmark & & 66.20 & 22.2 & 14.1 & 0.760 & 0.840 \\
\hline
(7) \method 				  & \checkmark & \checkmark & \checkmark & \checkmark & \textbf{66.30} & \textbf{22.5} & \textbf{14.7} & \textbf{0.755} & \textbf{0.834} \\
\hline
\end{tabular}}
\caption{Performance on several downstream tasks on Ego4D. StCC: State Change Classification~(\%). AR: Action Recognition~(\%). LTA: Long-term action anticipation. $\uparrow$: Higher is better. $\downarrow$: Lower is better.}
\label{tbl:ego4dmain}
\end{table}

==> tables/ek100_ablation.tex <==
\begin{table}[]
\centering
\begin{tabular}{l|cc|cc}
                                      & \multicolumn{2}{c|}{\textbf{Top-1 Accuracy (\%)}} & \multicolumn{2}{c}{\textbf{Top-5 Accuracy (\%)}} \\ \cline{2-5} 
                                      & \textbf{Verb}           & \textbf{Noun}           & \textbf{Verb}           & \textbf{Noun}          \\ \hline
\textbf{SSRL w/o CLR Loss}            &     -                    &   -                      &            -             &         -               \\
\textbf{SSRL w/o State Change Loss}   &                         &                         &                         &                        \\
\textbf{SSRL w/o AVID initialization} &                         &                         &                         &                        \\
\textbf{SSRL}                         &                         &                         &                         &        \\
\hline
\end{tabular}
% \vspace{0.5em}
\caption{}
\label{tbl:ek100ablation}
\end{table}

==> tables/ek100_main.tex <==
% \begin{table}[]
% \centering
% \begin{tabular}{l|cc|cc}
%                                      & \multicolumn{2}{c|}{\textbf{Top-1 Accuracy (\%)}} & \multicolumn{2}{c}{\textbf{Top-5 Accuracy (\%)}} \\ \cline{2-5} 
%                                      & \textbf{Verb}    & \textbf{Noun}    & \textbf{Verb}    & \textbf{Noun}   \\ \hline \hline
% \textbf{Scratch (Random weights)}    &      20.38            &   4.96               &   64.75               &       19.83          \\
% \textbf{AVID}                        &   26.62               &      9.00            &       69.79           &  25.50               \\
% \textbf{SSRL w/ random peaks}      &   28.71               &      8.33            &   73.17               &       27.29          \\
% \hline
% \textbf{SSRL w/ spectrogram peaks} &   \textbf{31.71}               &  \textbf{11.25}               &      \textbf{73.54}            &          \textbf{30.54}      \\
% \hline
% \end{tabular}
% \vspace{0.5em}
% \caption{Video action recognition accuracy on EPIC-KITCHENS-100}
% \label{tbl:ek100main}
% \end{table}


% \begin{table}[]
% \centering
% \normalsize
% \caption{}
% \label{table:main_results}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{c|cccc|cccc|cccc}
% \hline
% \textbf{} & \multicolumn{4}{c|}{\textbf{Overall}}  & \multicolumn{4}{c|}{\textbf{Unseen Participants}}                                                    & \multicolumn{4}{c}{\textbf{Tail Classes}}                                                           \\ \hline
% \textbf{}       & \multicolumn{2}{c}{\textbf{Top-1 Accuracy (\%)}} & \multicolumn{2}{c|}{\textbf{Top-5 Accuracy (\%)}} & \multicolumn{2}{c}{\textbf{Top-1 Accuracy (\%)}} & \multicolumn{2}{c|}{\textbf{Top-5 Accuracy (\%)}} & \multicolumn{2}{c}{\textbf{Top-1 Accuracy (\%)}} & \multicolumn{2}{c}{\textbf{Top-5 Accuracy (\%)}} \\ \hline
% \textbf{Method} & \textbf{Verb}           & \textbf{Noun}          & \textbf{Verb}           & \textbf{Noun}           & \textbf{Verb}           & \textbf{Noun}          & \textbf{Verb}           & \textbf{Noun}           & \textbf{Verb}           & \textbf{Noun}          & \textbf{Verb}           & \textbf{Noun}          \\ \hline
% \textbf{AVID}   &   25.88                     &        8.38                &                         &                         &                         &                        &                         &                         &                         &                        &                         &                        \\
% SSRL (without AVID weights)   &       27.21                 &      8.58                  &      71.21                   &     25.83                    &                         &                        &                         &                         &                         &                        &                         &    \\
% \textbf{SSRL (with AVID weights)}   &       \textbf{31.25}                 &      \textbf{9.58}                  &      \textbf{72.50}                   &     \textbf{27.38}                    &                         &                        &                         &                         &                         &                        &                         &                      
% \end{tabular}
% }
% \end{table}

% \begin{table}[h]
% \begin{tabular}{cccp{15mm}p{18mm}||cc|cc}
%               &                   &                   &                       &                            & \multicolumn{2}{c|}{\textbf{Top-1}} & \multicolumn{2}{c}{\textbf{Top-5}} \\ \hline
% \textbf{AVID~\cite{morgado2021audio}} & \textbf{CLR Loss} & \textbf{StC Loss} & \textbf{Random \newline Peaks} & \textbf{Spectrogram \newline Peaks} & \textbf{Verb1}        & \textbf{Noun1}       & \textbf{Verb5}       & \textbf{Noun5}       \\ \hline
%  \checkmark           &      \checkmark             &                   &                       &            \checkmark                &    29.92           &  9.67              &     73.33           &       29.54         \\
%  \checkmark             &                  &    \checkmark               &                       &  \checkmark                          &  29.29              &  10.46              &   70.58            &      29.00          \\
%               &    \checkmark               & \checkmark                &                       &     \checkmark                       &          25.75      &     8.12          &    71.25            &    27.29            \\
%               &                  &                   &                      &                           &    20.38            &    4.96            &       64.75         &    19.83           \\
% \checkmark          &                   &                   &                       &                  &     26.62           &     9.00           &    69.79            &      25.50        \\
% \checkmark          &   \checkmark                &                   &     \checkmark                 &                          &                &                &                &              \\
% \checkmark          &   \checkmark                &     \checkmark              &     \checkmark                 &                          &   28.71             &    8.33            &     73.17           &     27.29         \\
% \hline
% \checkmark          &   \checkmark                &     \checkmark              &                      &       \checkmark                   &    \textbf{31.71}            &    \textbf{11.25}            &     \textbf{73.54}           &      \textbf{30.54}        \\ 
% \hline
% \end{tabular}
% \vspace{0.5em}
% \caption{Video action recognition accuracy (\%) on EPIC-KITCHENS-100}
% \label{tbl:ek100main}
% \end{table}

\begin{table}[t]
\centering
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{|l|cccc|cc|cc|}
\hline
\multirow{2}{*}{\textbf{Method}} & 
\multirow{2}{*}{\textbf{$\Lavc$}} & 
\multirow{2}{*}{\textbf{$\Lastc$}} & 
\multirow{2}{*}{\thead{\textbf{MoI}\\\textbf{Sampling}}} & 
\multirow{2}{*}{\thead{\textbf{AVID}\\\textbf{Init}~\cite{morgado2021audio}}} & 
\multicolumn{2}{c|}{\textbf{Top1 Acc~$\uparrow$}} &
\multicolumn{2}{c|}{\textbf{Top5 Acc~$\uparrow$}} \\
&&&&& Verb & Noun & Verb & Noun \\ \hline
(1) Random        & & & &             					   & 20.38 & 4.96 & 64.75 & 19.83 \\
(2) AVID~\cite{morgado2021audio}          & & &  & \checkmark 					   & 26.62 & 9.00 & 69.79 & 25.50 \\
(3) \method w/o \avc          & & \checkmark & \checkmark & \checkmark & 29.92 & 10.46 & 70.58 & 29.00 \\
(4) \method w/o \loss          & \checkmark & & \checkmark & \checkmark & 29.29 & 9.67  & 73.33 & 29.54 \\
(5) \method w/o MoI & \checkmark & \checkmark & & \checkmark & 28.71 & 8.33  & 73.17 & 27.29 \\
(6) \method (scratch)     & \checkmark & \checkmark & \checkmark & & 25.75 & 8.12  & 71.25 & 27.29 \\
\hline
(7) \method 				  & \checkmark & \checkmark & \checkmark & \checkmark & \textbf{31.71} & \textbf{11.25} & \textbf{73.54} & \textbf{30.54} \\ 
\hline
\end{tabular}}
% \vspace{0.5em}
\caption{Action recognition on EPIC-Kitchens-100. Top1 and top5 accuracy (\%) is reported. $\uparrow$: Higher is better.}
% \vspace{-6mm}
\label{tbl:ek100main}
\end{table}


% \begin{table}[]
% \begin{tabular}{ccccc||cc|cc}
%      &          &          &              &                   & \multicolumn{2}{c|}{\textbf{Top-1 Accuracy}} & \multicolumn{2}{c}{\textbf{Top-5 Accuracy}} \\
% \multicolumn{1}{l}{AVID} & \multicolumn{1}{l}{CLR Loss} & \multicolumn{1}{l}{StC Loss} & \multicolumn{1}{l}{Random Peaks} & \multicolumn{1}{l||}{Spectrogram Peaks} & \multicolumn{1}{l}{Verb1} & \multicolumn{1}{l}{Noun1} & \multicolumn{1}{l}{Verb5} & \multicolumn{1}{l}{Noun5} \\ \\ \hline
%  \checkmark           &      \checkmark             &                   &                       &            \checkmark                &    29.92           &    9.67            &     73.33           &    31.54            \\
%  \checkmark             &                  &    \checkmark               &                       &  \checkmark                          &                &                &               &                \\
%               &    \checkmark               & \checkmark                &                       &     \checkmark                       &                &               &                &                \\
%               &                  &                   &                      &                           &                &                &                &               \\
% \checkmark          &                   &                   &                       &                  &                &                &                &              \\
% \checkmark          &   \checkmark                &                   &     \checkmark                 &                          &                &                &                &              \\
% \checkmark          &   \checkmark                &     \checkmark              &     \checkmark                 &                          &                &                &                &              \\
% \checkmark          &   \checkmark                &     \checkmark              &                      &       \checkmark                   &                &                &                &              \\
% \hline
% \end{tabular}
% \vspace{0.5em}
% \caption{Video action recognition accuracy on EPIC-KITCHENS-100}
% \label{tbl:ek100main}
% \end{table}


==> tables/supp_ego4d_keyframe.tex <==
\begin{table}[ht]
\centering
\resizebox{0.99\textwidth}{!}{
\begin{tabular}{|l|cccc|c|c|cc|}
\multicolumn{5}{c}{} & \multicolumn{1}{c}{\bf PNR} & \multicolumn{1}{c}{\thead{\bf StCC\\\bf w/ audio}}& \multicolumn{2}{c}{\thead{\bf AR \\\bf w/ Audio}}  \\ \hline
\multirow{2}{*}{\textbf{Method}} & 
\multirow{2}{*}{\textbf{$\Lavc$}} & 
\multirow{2}{*}{\textbf{$\Lastc$}} & 
\multirow{2}{*}{\textbf{MoI}} &
\multirow{2}{*}{\thead{\textbf{AVID}\\\textbf{Init}~\cite{morgado2021audio}}} & 
\multirow{2}{*}{\textbf{Err} $\downarrow$} &
\multirow{2}{*}{\textbf{Acc} $\uparrow$} &
\multicolumn{2}{c|}{\textbf{Top1 Acc} $\uparrow$} \\
&&&&&&& Verb & Noun \\\hline
\textcolor{lightgray}{(S1) I3D-ResNet-50~\cite{carreira2017quo, grauman2021ego4d}} & \textcolor{lightgray}{NA} & \textcolor{lightgray}{NA} & \textcolor{lightgray}{NA} & \textcolor{lightgray}{NA} & \textcolor{lightgray}{0.739} & \textcolor{lightgray}{-} & \textcolor{lightgray}{-} & \textcolor{lightgray}{-} \\
\textcolor{lightgray}{(S2) BMN~\cite{grauman2021ego4d, lin2019bmn}} & \textcolor{lightgray}{NA} & \textcolor{lightgray}{NA} & \textcolor{lightgray}{NA} & \textcolor{lightgray}{NA} & \textcolor{lightgray}{0.780} & \textcolor{lightgray}{-} & \textcolor{lightgray}{-} & \textcolor{lightgray}{-} \\
\hline
(1) Random        & & & &   						       &  0.827 & 52.90 & 18.90   & 9.50  \\
(2) AVID~\cite{morgado2021audio}          & & & & \checkmark  					   & 0.814 & 61.30 & 19.80 & 12.30  \\
(3) \method w/o \avc          & & \checkmark & \checkmark & \checkmark & 0.792 & 64.60 & 22.70 & 14.00 \\
(4) \method w/o \loss          & \checkmark & & \checkmark & \checkmark &  0.795 & 64.40 & 21.40  & 13.00  \\
(5) \method w/o MoI & \checkmark & \checkmark & & \checkmark & 0.801 & 64.10 & 20.80 & 11.70 \\
(6) \method (scratch)     & \checkmark & \checkmark & \checkmark & & 0.775 & 66.30 & 22.50 & 15.00 \\
\hline
(7) \method 				  & \checkmark & \checkmark & \checkmark & \checkmark & \textbf{0.772} & \textbf{66.80} & \textbf{23.10} & \textbf{15.80} \\
\hline
\end{tabular}}
\vspace{0.5em}
\caption{Performance on several downstream tasks on Ego4D. StCC: State Change Classification~(\%). PNR: Point-of-no-return temporal localization error~(seconds). AR: Action Recognition~(\%). $\uparrow$: Higher is better. $\downarrow$: Lower is better.}
\vspace{-5mm}
\label{tbl:supp_ego4d}
\end{table}

% \begin{table}[ht]
% \centering
% \resizebox{0.75\textwidth}{!}{
% \begin{tabular}{|l|cccc|c|} \hline
% \multirow{2}{*}{\textbf{Method}} & 
% \multirow{2}{*}{\textbf{$\Lavc$}} & 
% \multirow{2}{*}{\textbf{$\Lastc$}} & 
% \multirow{2}{*}{\textbf{MoI}} &
% \multirow{2}{*}{\thead{\textbf{AVID}\\\textbf{Init}~\cite{morgado2021audio}}} & 
% \multirow{2}{*}{\textbf{Acc} $\downarrow$} \\ 
% &&&&& \\\hline
% \textcolor{lightgray}{(S1) I3D ResNet-50~\cite{carreira2017quo, grauman2021ego4d}} & \textcolor{lightgray}{NA} & \textcolor{lightgray}{NA} & \textcolor{lightgray}{NA} & \textcolor{lightgray}{NA} & \textcolor{lightgray}{0.739} \\
% \textcolor{lightgray}{(S2) BMN~\cite{grauman2021ego4d, lin2019bmn}} & \textcolor{lightgray}{NA} & \textcolor{lightgray}{NA} & \textcolor{lightgray}{NA} & \textcolor{lightgray}{NA} & \textcolor{lightgray}{0.780} \\
% \hline
% (1) Random        & & & &   						       &  0.827 \\
% (2) AVID~\cite{morgado2021audio}          & & & & \checkmark  					   & 0.814 \\
% (3) \method w/o \avc          & & \checkmark & \checkmark & \checkmark & 0.792 \\
% (4) \method w/o \loss          & \checkmark & & \checkmark & \checkmark &  0.795 \\
% (5) \method w/o MoI & \checkmark & \checkmark & & \checkmark & 0.801 \\
% (6) \method (scratch)     & \checkmark & \checkmark & \checkmark & &  0.775 \\
% \hline
% (7) \method 				  & \checkmark & \checkmark & \checkmark & \checkmark & \textbf{0.772} \\
% \hline
% \end{tabular}}
% \vspace{0.5em}
% \caption{Performance on Point-of-no-return temporal localization error~(seconds) tasks on Ego4D, $\downarrow$: Lower is better.}
% \vspace{-5mm}
% \label{tbl:supp_ego4d}
% \end{table}

==> tables/unseen_head_tail.tex <==
% \begin{table}[h]
% \centering
% \footnotesize
% \resizebox{0.99\textwidth}{!}{
% \begin{tabular}{|l|cccc|cccc|cccc|}
% \hline
%                                      & \multicolumn{4}{c|}{\textbf{Unseen Participants}}                                        & \multicolumn{4}{c|}{\textbf{Head Classes}}                                               & \multicolumn{4}{c|}{\textbf{Tail Classes}}                                               \\ \cline{2-13} 
%                                      & \multicolumn{2}{c|}{\textbf{Top-1}}                & \multicolumn{2}{c|}{\textbf{Top-5}} & \multicolumn{2}{c|}{\textbf{Top-1}}                & \multicolumn{2}{c|}{\textbf{Top-5}} & \multicolumn{2}{c|}{\textbf{Top-1}}                & \multicolumn{2}{c|}{\textbf{Top-5}} \\ \cline{2-13} 
%                                      & Verb & \multicolumn{1}{c|}{Noun} & Verb    & Noun    & Verb & \multicolumn{1}{c|}{Noun} & Verb    & Noun    & Verb & \multicolumn{1}{c|}{Noun} & Verb    & Noun   \\ \hline
% AVID Weights                        &               & \multicolumn{1}{c|}{}              &                  &                  &     27.95          &  \multicolumn{1}{c|}{9.82}              &     73.20             &       28.43           &               & \multicolumn{1}{c|}{}              &   47.14              &  12.89               \\
% SSRL w/o MoI Sampling      &               & \multicolumn{1}{c|}{}              &                  &                  &               & \multicolumn{1}{c|}{}              &                  &                  &               & \multicolumn{1}{c|}{}              &                  &                 \\
% SSRL w/ MoI Sampling &               & \multicolumn{1}{c|}{}              &                  &                  &               & \multicolumn{1}{c|}{}              &                  &                  &               & \multicolumn{1}{c|}{}              &                  &         \\
% \hline
% \end{tabular}}
% \vspace{0.5em}
% \caption{Video action recognition accuracy (\%) on EPIC-KITCHENS-100 for unseen participants, head classes, and tail classes.}
% \label{tbl:ek100unseenheadtail}
% \end{table}

\begin{table}[h]
\resizebox{0.99\textwidth}{!}{
\begin{tabular}{|l|cccc|cccc|cccc|}
\multicolumn{1}{c}{} & \multicolumn{4}{c}{\textbf{Unseen Participants}} & \multicolumn{4}{c}{\textbf{Tail Classes}} & \multicolumn{4}{c}{\textbf{Head Classes}} \\ \hline
& \multicolumn{2}{c}{\textbf{Top1 Acc~$\uparrow$}} & \multicolumn{2}{c|}{\textbf{Top5 Acc~$\uparrow$}} & \multicolumn{2}{c}{\textbf{Top1 Acc~$\uparrow$}} & \multicolumn{2}{c|}{\textbf{Top5 Acc~$\uparrow$}} & \multicolumn{2}{c}{\textbf{Top1 Acc~$\uparrow$}} & \multicolumn{2}{c|}{\textbf{Top5 Acc~$\uparrow$}} \\
\bf Methods     & Verb  & Noun & Verb & Noun & Verb  & Noun & Verb  & Noun  & Verb  & Noun  & Verb  & Noun  \\ \hline
AVID~\cite{morgado2021audio}	    			&   26.17    & 8.67     &  68.75    &  24.12    & 16.80 & 4.43 & 47.14 & 12.89 & 27.95 & 9.82  & 73.20 & 28.43 \\
\method w/o \avc     &    28.67   & 9.38     & 72.04     & 27.88     & 18.49 & 5.21 & 47.79 & 12.63  & 30.59 & 10.21  & 73.33  & 30.90  \\
\method w/o MoI     &   27.71    &  7.92    &  72.08    &  26.88    & 16.80 & 4.04 & 49.74 & 12.76 & 29.36 & 10.65 & 76.33 & 30.41 \\
\hline
\method		&  \bf 31.58    & \bf 10.17      &  \bf 73.46    & \bf 29.96     & \bf 20.05 & \bf 6.12 & \bf 52.08 & \bf 16.54 & \bf 33.41 & \bf 11.58 & \bf 77.77 & \bf 34.33 \\ \hline
\end{tabular}}
\vspace{0.5em}
\caption{Video action recognition~(AR) accuracy (\%) on EPIC-Kitchens-100 for unseen participants, head classes, and tail classes. Top1 and top5 accuracy (\%) is reported. $\uparrow$: Higher is better.}
\vspace{-4mm}
\label{tbl:ek100unseenheadtail}
\end{table}
